Parameterized Verification of Systems with Global Synchronization and Guards

Inspired by distributed applications that use consensus or other agreement protocols for global coordination, we define a new computational model for parameterized systems that is based on a general global synchronization primitive and allows for global transition guards. Our model generalizes many existing models in the literature, including broadcast protocols and guarded protocols. We show that reachability properties are decidable for systems without guards, and give sufficient conditions under which they remain decidable in the presence of guards. Furthermore, we investigate cutoffs for reachability properties and provide sufficient conditions for small cutoffs in a number of cases that are inspired by our target applications.

==> GGBC.tex <==
\paragraph{Guarded Processes.} 
%\label{sec:extendedmodel}
Therefore, we introduce \emph{guarded} 
transitions that are only enabled if all processes are ready, i.e., they are in a 
specified subset $\guard \subseteq \LS$ of their local state space. $\guard$ 
is also called the \emph{guard} of the transition.

%\noindent \emph{Processes with guards.}
Formally, a \emph{(generalized) broadcast protocol with guards} is defined by 
a process of the form 
$\ph=\tuple{A,\LS,\ls_0,T}$, where all components are as before, except that 
now we have $T \subseteq \LS \times A \times \guards \times \LS$, i.e., 
transitions are additionally labeled with a subset of $\LS$, the guard. 
Wlog., we assume that matching output and input actions always have the same 
guard.
 
%\noindent \emph{Composition of processes with guards.}
Let the \emph{support} of a global state $\conf$ be $\supp(\conf) = \{ \ls \in \LS 
\mid \conf(\ls) > 0 \}$, i.e., the set of local states that appear at least 
once in $\conf$. %\nour{might need to extend this to also be over bags}
Then the semantics of a (generalized) broadcast transition on action $a$ with 
guard $G$, denoted $\trans{\conf}{a, \guard}{\conf'}$, is as defined before, 
except that the transition is enabled only if $\supp(\conf) \subseteq G$.

As an example, consider
\mn{\swen{add an example with guards}}
\mn{\nour{We can add guards to the examples above to simulate ``everyone in $G = \{c_1,c_2,np\}$ }}

\mn{\swen{mention that deadlocks can be checked by checking reachability of upwards-closed sets?}}

\paragraph{Modeling \ch with Generalized Broadcasts.}
\mn{\swen{we will not directly refer to \ch, but we may explain here how this allows us to model the motivating example}}
Note that multi-sender broadcasts allow us to model value-store agreement:
for every possible choice of $k$ winning values, we add a $k$-sender 
broadcast such that for each winning value, one sender needs to originate 
from a state that proposes the value. E.g., to model a $k$-sender broadcast 
for winning values $\{a,b\} \subseteq V$, add broadcast-sending transitions 
with action $\{a,b\}_1!!$ from every state that proposes $a$ to every 
possible post-state where $\{a,b\}$ has been selected, and broadcast-sending 
transitions with action $\{a,b\}_2!!$ from every state that proposes $b$ 
accordingly. Finally, the broadcast matrix $M_{\{a,b\}}$ moves all receiving 
processes to a state where $\{a,b\}$ has been selected.

Note further that maximal-sender broadcasts allow us to model agree-and-move agreement:
if $k$ winners should be chosen, add transitions with each of $a_1,\ldots,a_k$
 from every $c_i$ to the corresponding $w_i$.  If at least $k$ processes are 
present in the some combination of $c_i$ states,
then $k$ of them will move to their corresponding $w_i$. Otherwise, 
all of the processes in the $c_i$ states will move to their corresponding 
$w_i$. In any case, all 
other processes (those in the $c_i$ that are not senders and those in the non-
participating states) will move into the $l_i$ according to a broadcast 
matrix $M_a$.\\ 
\mn{\nour{In both cases we still need a guard on the transitions to make sure all participants are in the $c_i$ states. But otherwise, this seems reasonable.}}
%Then the parameterized system $\M_{GBC}(n)$ is defined as for broadcast protocols, except that
%transitions with action $a$ and guard $\guard$, written $\trans{\conf}{a, \guard}{\conf'}$, are only enabled if $\supp(\conf) \subseteq G$.

%In order to define the global transition $\trans{\conf}{a}{\conf'}$, we introduce some notation. Let:
%\begin{itemize}
%\item $M_a$ be a broadcast matrix such that $M_a(\ls_j,\ls_i) = 1$ if $\trans{\ls_i}{a??}{\ls_j} \in T$. All other entries of $M_a$ are $0$.
%\nour{\\Yes, this looks bad but we can massage it later:}
%\item $K^{in}_a: S \rightarrow \Nats$ be defined as $$K^{in}_a(\ls) =\sum_{\{ k ~\mid~ \trans{\ls'}{a!!k}{\ls} \ \in T \}} k$$
%% $K_{in}(\ls) =\sum_{\{ s' \in S_a ~\mid~ \trans{\ls'}{a!!k}{\ls} \ \in T \}} K_a(s')$
%\item $K^{no}_a: S \rightarrow \Nats$ be defined as $$K^{no}_a(\ls) =\sum_{\{ k ~\mid~ \trans{\ls'}{a!!k}{\ls''} \ \text{and} \ \trans{\ls'}{a??}{\ls} \ \in T \}} k$$
%%$K_{no}(\ls) =\sum_{\{ s' \in S_a ~\mid~ \trans{\ls'}{a!!k}{\ls''} \ \text{and} \ \trans{\ls'}{a??}{\ls} \ \in T\ \text{with} s'' \neq s\}} K_a(s')$
%\item $V_a$ be a broadcast vector such that: $$\forall s \in S, V_a(s) = K^{in}_a(s) - K^{no}_a (s).$$
%\item $S_a = \{\ls_i \mid \trans{\ls_i}{a!!k}{\ls_j}\ \in T\}$ where $k \in \Nats$ be the set of states with an outgoing broadcast-send label.
%\item $\card_a: S_a \rightarrow \Nats$ be a function mapping each state $\ls$ in $S_a$ to a number $k$ that appears on the broadcast-send transition originating from $\ls$, i.e. $\trans{\ls}{a!!k}{\ls'}\ \in T$. 
%\end{itemize}
%Informally, the broadcast matrix moves the receiving processes from their current state to the next state upon receiving a broadcast. The broadcast vector essentially ``adjusts'' the states of the senders who would have moved with the receivers. 
%
%\noindent{\em Enabledness of multi-sender broadcasts.} Note a multi-sender broadcast $a$ is only enabled in a global state $\conf$ if the following condition holds:
%$$\forall \ls \in S_a, \conf(\ls) \ge \card(\ls)$$
%
%%In other words, each broadcast-send state $\ls$ must have at least $k$ processes.
%
%Finally, if a multi-sender broadcast $a$ is enabled in global state $\conf$ then $\trans{\conf}{a}{\conf'} \in Q$ and $\conf' = M_a \cdot \conf + V_a$.
%
%Essentially, for each transition $\trans{\ls}{a!!k}{\ls'}$, exactly $k$ processes move from state $\ls$ to state $\ls'$ and for each transition $\trans{\ls}{a??}{\ls'}$, all processes move from state $\ls$ to state $\ls'$.
%
%
%
%
%
%
%
%
%
%\nour{Skip this for now, might be useful for the mapping!\\}
%\begin{itemize}
%%\item $S_a = \{\ls_i \mid \trans{\ls_i}{a!!k}{\ls_j}\ \in T\}$ where $k \in \Nats$ be the set of states with an outgoing broadcast-send label.
%\item $D_a = \{\ls_j \mid \trans{\ls_i}{a!!k}{\ls_j}\ \in T\}$ be the set of states with an incoming broadcast-send label.
%\item $Z_a = \{\ls_h \mid \trans{\ls_i}{a!!k}{\ls_j}$ and $\trans{\ls_i}{a??}{\ls_h}\ \in T\}$ be the set of states where the senders would have transitioned if they took the broadcast-receive edge instead.
%\item $\Succ_a : S_a \rightarrow D_a$ be function mapping a state $\ls_i \in S_a$ to a state $\ls_j \in D_a$ such that $\trans{\ls_i}{a!!k}{\ls_j}\ \in T$.
%\item $\FalseSucc_a : S_a \rightarrow Z_a$ be function mapping a state $\ls_i \in S_a$ to a state $\ls_h \in Z_a$ such that $\trans{\ls_i}{a!!k}{\ls_j}$ and $\trans{\ls_i}{a??}{\ls_h}\ \in T$.
%%\item $\card_a: S_a \rightarrow \Nats$ be a function mapping each state $\ls$ in $S_a$ to a number $k =\card(\ls)$. 
%\end{itemize}
%
%
%
%
%
%
%
%
%
%\subsection{The Smoke Detector Example in this Model}
%\edit{make sure we refine this to match the new intro example.}
%%\resizebox{\textwidth}{!}{\includegraphics{example.png}}
%\input{smokemodel}
%To clarify the relation to the previous model, let us consider again the smoke detector in~\figref{introExample}. First, note that the transition from $Env$ to $Init$ sets a local variable. Since in this model we do not keep track of local variables, this means we have to split into two different states. Then, note that states $Init$, $Wait$ and $Store$ are used to synchronize all processes, i.e., every process can only leave $Wait$ into $Idle$ or $Pick$ if it has heard from all other processes. For parameterized verification, we summarize the synchronization of process into a single negotiation step, i.e., a broadcast that does not have a dedicated sender, but all nodes simultaneously take a transition according to their current local state\footnote{Systems that only communicate through negotiation have been investigated by \citet{ED13}.}: from $Wait_2$, the process moves to $Pick$, and from $Wait_1$ to $Idle$. To ensure that this can only happen if all processes are ready, we add a guard that requires all processes to be in either $Wait_1$ or $Wait_2$ for this transition to be enabled. Then, the \ch(2) can be modeled by a sequence of two broadcast transitions, which we summarize in a single transition that takes $2$ processes to $Rep.$ and all other processes that are in $Pick$ to $Idle$, as shown in~\figref{smoke-sensors-param}.



%We have a chain of $k$ broadcasts on action ``choose'', to ensure that exactly $k$ processes can move to ``win''. For the case where less than $k$ processes are available for ``choose'', consider a system with the following changes:
%\begin{itemize}
%\item state ``win'' is a part of $C$, i.e., $C=\{c_1,c_2,win\}$
%\item all states where a choose transition is possible have additional transitions to the initial state, which are guarded with $\forall C$. When these transitions to the initial state are taken, the process has to remember how many choose actions it has already taken and enter the line of choose operations in the right place when the next ``done'' is taken.
%\end{itemize}
%
%\nour{why are we adding this last point? are we supporting a system where < k win and the rest are still in detect, trying to enter the critical section with whatever remaining capacity? e.g.  capacity = 5, 2 enter win, the rest of processes fight over the 3 spots?}
%\roopsha{Perhaps add this as a note that it could be done?}

%\input{gbcp} %async. transitions to the GBC model.
%\input{gbcp_verification}
%\input{chooseflavors}

==> Implementation.tex <==
\section{Implementation}
\label{sec:implementation}


==> PV2_with_Weak_GC.tex <==
\section{Parameterized Verification for GSPs with Guards}
\label{sec:PV-guards}
%%
%Esparza et al.~\cite{EsparzaFM99} have defined the following WQO on the (global) states of the basic model of broadcast protocols:
%
%$$\conf \wqo \conf' \text{ iff }\conf(\ls) \leq \conf'(\ls) \text{ for all } \ls \in \LS.$$
%
%%, and one of the following holds:
%%\begin{enumerate}
%%\item $c_1=c_2=c_1'=c_2'=0$ and $\sum_{q \notin Q_c} \conf(q) > 0 < \sum_{q \notin Q_c} \conf'(q)$, 
%%\item $c_1=c_2=c_1'=c_2'=0$ and $\sum_{q \notin Q_c} \conf(q) = 0 = \sum_{q \notin Q_c} \conf'(q)$,
%%\item $c_1>0<c_1'$, $c_1 \geq c_2$ and $c_1' \geq c_2'$, or
%%\item $c_2>0<c_2'$, $c_1 < c_2$ and $c_1' < c_2'$.
%%\end{enumerate}
%%Note that the well quasi order is only partially defined, and it is undefined for almost all pairs of states in instances of the same size: $\conf(q) \leq \conf'(q)$ for all $q \in Q$ can only hold if the instance of $\conf'$ is at least as big as the instance of $\conf$, and if their size is equal it can only hold if $\conf(q)=\conf'(q)$ for all $q$.
%
%Based on this, they have shown:
%\begin{theorem}[\cite{EsparzaFM99}]
%\label{thm:compatibility}
%For the model of broadcast protocols and the WQO above, the following hold:
%\begin{itemize}
%\item Broadcast transitions are \emph{strongly compatible} with the WQO, i.e., if $\conf \wqo \conf'$ and $\conf \rightarrow \altconf$, then $\exists \altconf'$ with $\altconf \wqo \altconf'$ and $\conf' \rightarrow \altconf'$. This implies that for a given upward-closed set of states $C$, the set of predecessor states $Pred(C)$ is also upward-closed.\footnote{In fact, Esparza et al. have only proven the latter, but one can show that the two statements are equivalent.}
%\item For broadcast transition systems we can effectively compute Pred. 
%\end{itemize}
%\end{theorem}
%
%We quickly recapitulate their proof idea, because it will inform our proof for guarded broadcast protocols.
%
%\begin{proof}
%For both items, it is sufficient to show them for every action $a \in A$ separately. With our formulation, the first item is easy to show based on the matrix notation of broadcast transitions. For the second, observe that for a transition based on $\trans{\ls_k}{a!!}{\ls_l}$, any element $\conf$ of $Pred(C)$ must satisfy $\conf(\ls_k) \geq 1$ and $M_a \cdot \conf + \mathbf{v}_a = \conf'$, for some $\conf' \in C$. The basis of $Pred(C)$ consists of the minimal elements that satisfy these conditions, and thus is computable.
%\end{proof}
%
%In our setting, $\conf \preceq \conf'$ means that $\conf$ is a global state 
%of $\M(n)$, $\conf'$ is a global state of $\M(n')$ with $n' \geq n$, and the 
%two states are similar in a way that preserves certain properties, e.g. that 
%for every transition $\trans{\conf}{a}{\altconf}$ there is also a transition 
%$\trans{\conf'}{a}{\altconf'}$.
%If $\preceq$ is also compatible with the 
%transition relation, then we further know that $\altconf \preceq \altconf'$ 
%(or that such a $\altconf'$ can be reached after multiple transitions), 
%i.e., this similarity of states is carried over transitions, and 
%therefore allows us to decide reachability problems for arbitrarily large 
%systems by reasoning about small representatives.
%
For GSPs with guards, compatibility under $\wqo$ in general 
does not hold, since for $\conf \wqo \altconf$, it might be that a transition 
on action $a$ that is enabled in $\conf$ is not enabled in $\altconf$.
\new{Furthermore, note that even strong restrictions on processes are unlikely to yield 
compatibility with respect to $\wqo$, since for any given $\conf$ where a non-trivial guard $\guard \neq \LS$ is enabled, one can always find a $\altconf$ 
with $\conf \wqo \altconf$ where $\guard$ is disabled, i.e., such that $\altconf(\ls) > 0 $ for some local state $\ls \notin \guard$. 
}
\mn{old: Furthermore, note that even strong restrictions on processes are unlikely to yield compatibility with respect to $\wqo$, since for any given $\conf$ that 
satisfies a non-trivial guard $\guard \neq \LS$ one can always find a $\altconf$ 
with $\conf \wqo \altconf$ such that $\altconf$ does not satisfy $\guard$, i.e., such that $\altconf(\ls) > 0 $ for some local state $\ls \notin \guard$.} 

Therefore, we introduce a refined WQO, denoted $\altwqo$, that is based on the semantics of 
guards, as well as sufficient conditions on the guarded process $P$, 
such that the system $\M_\infty$ is a WSTS and we can effectively compute $
Pred$.

Let $\mathcal{G}$ be the set of guards that appear on transitions in $P$, and recall that $\supp(\conf) = \{ \ls \in \LS \mid \conf(\ls) > 0 \}$. 
Then we consider the following WQO\footnote{\new{To see that 
this is really a WQO, we need to show that every infinite sequence $\conf_1, 
\conf_2, \ldots$ of global states contains contains $\conf_i, \conf_j$ with $i
<j$ and $\conf_i \altwqo \conf_j$. To see this, consider an arbitrary infinite 
sequence $\overline{\conf} = \conf_1, \conf_2, \ldots$. Then there is at 
least one set $S$ of local states such that there are infinitely many 
$\conf_i$ with $\supp(\conf_i)=S$. Then let $\overline{\conf'}$ be the 
infinite 
subsequence of $\overline{\conf}$ where all elements have $\supp(\conf'_i)=S$. 
Since $\wqo$ is a WQO, there exist $\conf'_i, \conf'_j$ with $i<j$ and 
$\conf'_i \wqo \conf'_j$, and since $\supp(\conf'_i)=\supp(\conf'_j)=S$, we 
also get 
$\conf'_i \altwqo \conf'_j$. Since $\conf'_i = \conf_k$ and $\conf'_j = \conf_l$
 for some $k < l$, we get $\conf_k \altwqo \conf_l$ for $k < l$, and thus 
$\altwqo$ is a WQO.}}:
%\mn{\swen{need to show that this is a WQO?}}
%\footnote{To see that 
%this is really a WQO, we need to show that every infinite sequence $\conf_1, 
%\conf_2, \ldots$ of global states contains contains $\conf_i, \conf_j$ with $i
%<j$ and $\conf_i \altwqo \conf_j$. To see this, consider an arbitrary infinite 
%sequence $\overline{\conf} = \conf_1, \conf_2, \ldots$. Then there is at 
%least one set $S$ of local states such that there are infinitely many 
%$\conf_i$ with $\supp(\conf_i)=S$. Then let $\overline{\conf'}$ be the 
%infinite 
%subsequence of $\overline{\conf}$ where all elements have $\supp(\conf'_i)=S$. 
%Since $\wqo$ is a WQO, there exist $\conf'_i, \conf'_j$ with $i<j$ and 
%$\conf'_i \wqo \conf'_j$, and since $\supp(\conf'_i)=\supp(\conf'_j)=S$, we 
%also get 
%$\conf'_i \altwqo \conf'_j$. Since $\conf'_i = \conf_k$ and $\conf'_j = \conf_l$
% for some $k < l$, we get $\conf_k \altwqo \conf_l$ for $k < l$, and thus 
%$\altwqo$ is a WQO.}
$$\conf \altwqo \altconf \; \text{ iff } \; \left( \conf \wqo \altconf \land \forall \guard \in \mathcal{G}: \left( \supp(\conf) \subseteq \guard \iff \supp(\altconf) \subseteq \guard \right) \right).$$

\mn{this is still true with the ``iff'' maybe let's keep it as is?}The intuition behind the WQO is that a global state $\altconf$ is considered 
greater\mn{bigger?} than a global state $\conf$ if $\altconf$ has at least as many 
processes as $\conf$ in any given state, \emph{and} for every transition 
$\trans{\conf}{a}{\conf'}$ that is enabled in 
$\conf$, a transition on action $a$ is also enabled in $\altconf$. 

We will see that compatibility with respect to $\altwqo$ can only be ensured under 
additional conditions, as formalized in the following.
%We note that this requirement essentially states that the parameterized system moves in rounds (if one thinks of each broadcast as a round), and that the boundaries of such rounds (i.e. where those broadcasts are enabled or disabled) is independent of the specific instantiation of the parameterized system.}

\subsection{Guard-Compatibility and Well-Behaved Processes}
\label{sec:well-behavedness}
We start by defining the notion of strong guard-compatibility, which implies strong compatibility of transitions with respect to $\altwqo$. Then, we relax our conditions to weak guard-compatibility, which only implies compatibility w.r.t. $\altwqo$.

\paragraph{Strong Guard-Compatibility for $k$-Sender Actions.}
For a $k$-sender action $a$, let $\senderset$ be the set of states $\ls_i$ 
such that $\trans{\ls_i}{a_i!!, \guard}{\ls_i'}$, $1 \leq i \leq k$, are the 
local sending transitions, $\senderset'$ the set of all states $s_i'$, and 
$M_a$ the synchronization matrix. 
We say that action $a$ is 
\emph{strongly guard-compatible} if the following holds for all $\guard' \in \guardset{
:}$

%\left(\senderset \subseteq \guard' \land \senderset' \subseteq \guard' 
%\Rightarrow \forall \ls \in \guard{:}~ \left(\ls \in \guard' \Rightarrow M_a(
%\ls) \in \guard'\right) \right)\\
%\land \left(\senderset \not \subseteq \guard' \land 
\[ 
\senderset' \subseteq \guard' \Rightarrow \forall \ls \in \guard{:}~ M_a(\ls) \in \guard' 
\tag{C1} \label{eq:guard-comp-k-sender}
\]
%\right)

Intuitively, if all senders move into a guard $\guard'$, then also all 
receivers need to move into $\guard'$. This ensures that if $\guard'$ is satisfied after the transition in a system of a given size, then it is satisfied after that transition in a system of any bigger size, because any additional receivers must also move into $\guard'$. \new{Note that Condition~\eqref{eq:guard-comp-k-sender} always holds for trivial guards.}


%Furthermore, note that negotiation actions are a special case with $k=0$. Because there are no senders, the premise of ~\eqref{eq:guard-comp-k-sender} always holds, so negotiations are strongly guard-compatible only when all associated receive transitions end within (or outside of) the same guards.

%\mn{\swen{need the special case for rendezvous?}}
%For the special case of rendezvous transitions (where $k=2$ and $M_a=Id$), 
%$\trans{\ls_i}{a_1!!, \guard}{\ls_i'}$ 
%and $\trans{\ls_j}{a_2!!, \guard}{\ls_j'}$, we get that action $a$ is \emph{guard-compatible} if 
%for all $\guard' \in \mathcal{G}$:

%\[
%\left( \left( 
%\ls_i' \in \guard' \land \ls_j' \in \guard'\right) \Rightarrow 
%\left( \guard \subseteq \guard' \right) \right)
%\tag{C1a} \label{eq:guard-comp-rendezvous}
%\]

\paragraph{Strong Guard-Compatibility for $k$-Maximal Actions.}
For a $k$-maximal action $a$, the idea of the condition is the same as 
before, but it must be extended to allow different subsets of the 
\emph{potential} senders to act as \emph{actual} senders in a given transition with 
action $a$.
A simple approximation is that all senders must agree, for every $\guard \in 
\guardset$, on whether they enter $\guard$ or not.

In the following, we formalize a more refined notion that also takes into 
account that a transition that only uses a subset of the potential senders is 
only possible from certain global states, and that global states with 
different sets of actual senders may be incomparable with respect to 
$\altwqo$, and therefore unproblematic for compatibility.

We write $t \triangleleft \ls$ if, for all guards $\guard \in \guardset$, $s 
\in \guard \Rightarrow t \in \guard$. Similarly, we write $t \triangleleft H$ for a set of states $H$ if, for all guards $\guard \in \guardset$, $H \subseteq \guard \Rightarrow t \in \guard$.

Consider a $k$-maximal action $a$ with local transitions $\trans{\ls_i}{a_i!!,G
}{\ls_i'}$ for $i \in \{1,\ldots,k\}$ and synchronization matrix $M_a$. Let $R
= G \setminus \{s_1,\ldots,s_k\}$ and let $\guardset'$ be the set of all 
guards $\guard_R \in \guardset$ such that $R \subseteq \guard_R$.

Then we say the action $a$
is \emph{strongly guard-compatible} if both of the following hold for all $\guard' \in \guardset{
:}$
\[
\left(\bigvee_{1 \leq i \leq k} \ls_i' \in \guard' \right) \Rightarrow \left( \forall \ls \in R: M_a(\ls) \in \guard' \right)
\tag{C2.1} \label{eq:guard-comp-k-max-1}
\]
\[
\bigwedge_{i,j \in \{1,\ldots,k\}} \left( (\ls_i \triangleleft \ls_j \land \ls_j' \in \guard') \Rightarrow (\ls_i' \in \guard' \land M_a(\ls_i) \in \guard')
\right)
\tag{C2.2} \label{eq:guard-comp-k-max-2}
\]

Intuitively, if one potential sender moves from a state $\ls_j$ into a guard $\guard'$, then every 
receiver from $R$ must do the same, so that $\guard'$ will be satisfied regardless of the number of receivers. This is also required for other senders and receivers 
from a state $\ls_i \notin R$, unless there exists a guard that is satisfied 
if $\ls_j$ is occupied, but not if $\ls_i$ is occupied, since that means that a global state where only $\ls_j$ is occupied is incomparable (w.r.t. $\altwqo$) to a state where also $\ls_i$ is occupied, and therefore we do not care about compatibility of the transitions. 

Note that for $k=1$, the first condition~\eqref{eq:guard-comp-k-max-1} instantiates to 
condition~\eqref{eq:guard-comp-k-sender} and the second condition~\eqref{eq:guard-comp-k-max-2} is an empty 
conjunction, 
i.e., vacuously satisfied. This is to be expected, since semantically there 
is no difference between a $1$-sender action and a $1$-maximal action.

\begin{example}
We can see that actions \tr{\Smoke}, \tr{\Choose}, and \tr{\Resett} from our motivating example in \figref{MappedIntroExample} are strongly strongly guard-compatible:
\begin{compactenum}[--]

\item \tr{\Smoke} is a 1-sender action with sending transition \trans{\st{\Ask}}{\trr{\Smoke}!!, \{\st{\Env, \Ask}\}}{\st{\Pick}}. The state \st{\Pick} is only included in one non-trivial guard $G_2$ = \{\st{\Pick}, \st{\Idle}\}. Since receiving transitions from \{\st{\Env, \Ask}\} end in $\{\st{\Pick, \Idle}\} \subseteq G_2$, condition~\eqref{eq:guard-comp-k-sender} holds, so \tr{\Smoke} is strongly guard-compatible.

\item Consider \tr{\Choose} with sending transitions $\trans{\st{\Pick}}{\trr{\Choose_i!!},\{\st{\Pick,\Idle}\}}{\st{\Report}}$ for $i \in \{1,2\}$ as a 2-sender action. \st{\Report} is only included in one non-trivial guard $G_3$ = \{\st{\Report}, \st{\Idle}\}. Since the receiving transition from \{\st{\Pick}\} ends in $\st{\Idle} \in G_3$ as well,~\eqref{eq:guard-comp-k-sender} holds, so \tr{\Choose} is strongly guard-compatible.


%\item Consider \tr{\Choose} with sending transitions $\trans{\st{\Pick}}{\trr{\Choose_i!!},\{\st{\Pick,\Idle}\}}{\st{\Report}}$ for $i \in \{1,2\}$ as a 2-sender action. \st{\Report} is only included in one non-trivial guard $G_3$ = \{\st{\Report}, \st{\Idle}\}. Since the receiving transition from \{\st{\Pick}\} ends in $\st{\Idle} \in G_3$ as well,~\eqref{eq:guard-comp-k-sender} holds, so \tr{\Choose} is strongly guard-compatible.
\item \new{\mn{not very informative and will be really long if made detailed??}Consider \tr{\Choose} as a 2-maximal action. Again, \st{\Report} is only included in one non-trivial guard $G_3$ = \{\st{\Report}, \st{\Idle}\}. Since all senders and receivers start from \st{\Pick} and end up in a state in $G_3$, conditions \eqref{eq:guard-comp-k-max-1} and \eqref{eq:guard-comp-k-max-2} hold and \tr{\Choose} is, again, strongly guard-compatible.}





%\item Consider \tr{\Choose} as a 2-maximal action. Conditions \eqref{eq:guard-comp-k-max-1} and \eqref{eq:guard-comp-k-max-2} are implied by~\eqref{eq:guard-comp-k-sender}, so because~\eqref{eq:guard-comp-k-sender} holds, \tr{\Choose} is, again, strongly guard-compatible.




% in the 2-sender case, because both sending actions move from $\st{\Pick}$ to $\st{\Report}$. \st{\Report} is only included in one non-trivial guard $G_3$ = \{\st{\Report}, \st{\Idle}\}. Because the receiving transition from \{\st{\Pick}\} ends in $\st{\Idle} \in G_3$ as well, condition~\eqref{eq:guard-comp-k-sender} is satisfied. 


%, and for non-trivial guards this action trivially satisifes conditions \eqref{eq:guard-comp-k-max-1} and \eqref{eq:guard-comp-k-max-2} by negating the premises of all implications (and for the trivial guard $\guard=\LS$ all the consequences are trivially satisfied).

\item \tr{\Resett} is a negotiation action. Recall that negotiations are modeled as a set of 1-sender actions, allowing for an arbitrary sender. Therefore, each of these broadcasts must satisfy~\eqref{eq:guard-comp-k-sender} for the negotiation to be guard-compatible.
\tr{\Resett} is indeed strongly guard-compatible because all of its sending and receiving transitions end in the \st{Env} state, meaning that when the action fires, all processes will move into a single state, ensuring that all guards will be uniformly enabled or disabled, regardless of the number of processes, which of them is the sender, or whether they begin in \st{Report} or \st{Idle}.
%as a 2-maximal action with sending transitions $\trans{\st{\Pick}}{\tr{\Choose_i},\{\st{\Pick,\Idle}\}}{\st{\Report}}$ for $i \in \{1,2\}$. \st{\Report} is not included in any non-trivial guard, so for non-trivial guards this action trivially satisifes conditions \eqref{eq:guard-comp-k-max-1} and \eqref{eq:guard-comp-k-max-2} by negating the premises of all implications (and for the trivial guard $\guard=\LS$ all the consequences are trivially satisfied).
\end{compactenum}
\end{example}

\paragraph{Refinement: Weak Guard-Compatibility.} 
To support a larger class of transitions, we show how to relax the previous 
conditions, at the cost of making them more complex. 
The idea is that, instead of requiring that any guard that is 
satisfied by the senders is also satisfied by the receivers immediately after 
the transition, it is enough if 
the receivers \emph{have a path} to a state that satisfies all these guards. To 
avoid unnecessary complexity, we only consider paths of internal transitions.


If there exists a path of unguarded internal transitions from $\ls$ to $\ls'$, we write 
$\ls \rightsquigarrow \ls'$.
Then, condition~\eqref{eq:guard-comp-k-sender} can be relaxed to
\[ 
\senderset' \subseteq \guard' \Rightarrow \forall \ls \in \guard{:}~ \left( M_a(\ls) \in \guard' \lor \exists \ls' \in \LS: (\ls' \triangleleft \senderset' \land M_a(\ls) \rightsquigarrow \ls') \right) 
\tag{C1w} \label{eq:guard-comp-k-sender-weak}
\]

In a similar way, conditions~\eqref{eq:guard-comp-k-max-1} can be relaxed to obtain condition (C2.1w)  by replacing $M_a(\ls) \in \guard'$ with $M_a(\ls) \in \guard' \lor \exists \ls' \in \LS: (\forall \ls_i': (\ls' \triangleleft \ls_i') \land M_a(\ls) \rightsquigarrow \ls')$, and (C2.2w) is obtained from \eqref{eq:guard-comp-k-max-2} by replacing $M_a(\ls_i) \in \guard'$ with $M_a(\ls_i) \in \guard' \lor \exists \ls' \in \LS: (\ls' \triangleleft \ls_i' \land M_a(\ls_i) \rightsquigarrow \ls')$.
 
Actions that satisfy condition \eqref{eq:guard-comp-k-sender-weak} or (C2.1w) and (C2.2w) are called \emph{weakly guard-compatible}.
%\mn{\swen{not sure if this is needed:}}
%Note that it is in general not enough to require that $t'$ satisfies $\guard'$: since we are quantifying over all guards in our condition, the weaker condition might be satisfied if there are different paths to different states $t'$ that individually satisfy one guard that $\ls'$ satisfies, but still no path to a global state $\altconf'$ with $\conf' \altwqo \altconf'$.

\paragraph{Refinement: Internal Transitions.}
For internal transitions, we can relax the condition a bit further. Intuitively, since all receiving processes stay in their current state, it is enough to require condition (C1w) to hold if a guard is satisfied after the transition that was not satisfied before. Furthermore, the internal transitions that the ``receivers'' can use to reach a state that satisfies the same guards as the sender can be guarded, as long as the guard is general enough to guarantee that these transitions can be taken.\footnote{Guarding these internal transitions is also possible with more complicated conditions in other cases, but for simplicity we only introduce it formally for internal transitions.}

%\footnote{In fact, guarding these internal transitions is also possible under more complicated conditions in other cases, but for simplicity we only introduce it formally for internal transitions.}

Formally, we write $\ls \rightsquigarrow_G \ls'$ if there exists a path of internal transitions from $\ls$ to $\ls'$ such that each transition is guarded by some $\guard' \supseteq \guard$. Then, we say that an internal action $a$ is \emph{weakly guard-compatible} if
the following holds for every $\guard' \in \guardset$ (note that $\senderset$ 
and $\senderset'$ are both singleton sets, denoted $\ls$ and $\ls'$ in the 
following) and every $t \in \guard$:
\[
\ls \notin \guard' \land \ls' \in \guard' \Rightarrow \exists t':~ (t' \triangleleft \ls' \land t\rightsquigarrow_{\guard''} t'),
\tag{C3w} \label{eq:guard-comp-internal}
\]
where $\guard'' = \guard \cup \{ t \mid t \triangleleft \ls'\}$.

\begin{example}
We observe that the internal transition %\mn{\swen{do we need an action name?}} 
$\trans{\st{\Env}}{}{\st{\Ask}}$ from our motivating example in \figref{MappedIntroExample} is weakly guard-compatible, since there is no guard in the system that includes \st{\Ask}, but not \st{\Env}, so the premise of~\eqref{eq:guard-comp-internal} is negated.

%\mn{we can probably leave this out? \swen{leave out if we need space}}Moreover, if we consider a modified example where $\trr{\Resett}$ is ``split'' into two internal transitions that are guarded by $\guard_3' = \{\st{\Report, \Idle, \Env, \Ask}\}$, then both of these transitions are also weakly guard-compatible: they do move into $\guard_1$, which is not satisfied by their respective pre-state, but from every state in $\guard_3'$ there is a path of internal transitions that ends in a state that satisfies all guards that are satisfied by $\st{\Env}$ (namely, $\st{\Env}$ itself), and all transitions on this path are guarded by $\guard_3'$, which includes the guard of the internal transition under consideration ($\guard_3'$ itself), as well as the post-state of the transition.
\end{example}

%Intuitively, what condition~\eqref{eq:guard-comp-internal} requires is that if an internal transition crosses a guard boundary such that the guard is now satisfied by that process, then other processes that do not satisfy the guard also need to have a path of internal transitions to a local state that satisfies the same guards.

%\mn{\swen{use something like the following or not?}}
%Note that we require the existence of a single transition $\trans{t}{b_1!!, 
%\guard''}{t'}$, even though for compatibility it would be enough to have 
%$t \rightarrow^* t'$. We assume that in our protocols multiple subsequent 
%internal transitions are always summarized into a single transition, and 
%therefore this is not a major restriction.


\paragraph{Well-Behavedness.}
Having defined guard-compatibility for different types of actions, we can now 
define the type of processes that will allow us to retain decidability of 
reachability properties in the parameterized system:
We say that a process $P$ is \wellbehaved if every action is (weakly) guard-compatible.

Note that unguarded processes are trivially well-behaved.

\input{wellbehavnessExample}

\paragraph{Well-Behaved Systems in the Literature.}
We want to point out that many systems studied in the literature are naturally well-behaved.

For example, Emerson and Kahlon~\cite{EK03a} introduce a model for cache 
coherence protocols that is based 
on broadcast communication and guards. They show that many textbook protocols 
can be modeled under the following restrictions:
(i) every state is assumed to have an unguarded internal transition to the 
initial state $\st{Init}$, and (ii) the only (conjunctive) guard is 
$\{ \st{Init} \}$. Clearly, every action in a process that satisfies these 
conditions will also satisfy condition~\eqref{eq:guard-comp-k-sender-weak}, 
and therefore well-behaved systems subsume and significantly generalize 
the types of protocols considered by Emerson and Kahlon. 

Moreover, there has recently been much research on the verification of round-based distributed systems~\cite{Gleissenthall.Pretend.Synchrony.POPL.2019,damian.communicationclosed.CAV.2019,choosepaper.arxiv}, where processes can move 
independently to some extent, with the restriction that transitions between rounds
can only be done synchronously for all processes. When abstracting from certain features (e.g. fault-tolerance and process IDs), our model is well-suited to express such 
systems: guards can be used to restrict transitions to happen only in a 
certain round, and can furthermore model the ``border'' of a round that needs 
to be reached by all processes, such that they can jointly move to the next 
round.

Our example from \figref{MappedIntroExample} can also be seen 
as a round-based system: the first round includes states $\st{\Env, \Ask}$, and 
upon taking the transition on $\trr{\Smoke}$, all processes move to the second 
round, which includes states $\st{\Pick, \Idle}$. From there, on action 
$\trr{\Choose}$ the system moves to the third round, which includes states 
$\st{\Report, \Idle}$, and on action $\trr{\Resett}$ back to the first round. 
Note that the states in different rounds are exactly the guards that are used 
in the transitions---or seen the other way around, guards induce a set of 
rounds on the local state space, and the guard-compatibility conditions 
ensure that processes move between these rounds in a systematic way.

While the rounds are very simple in this example, the technique is much more 
general and can be used to express many round-based systems, including 
those described in~\secref{evaluation}.

%Naturally, the design of these systems ensures that when an action is sent, then all other processes are in phases

%If a specific action can be sent in round x, then all other processes can receive it during that round.

%There is an expected set of input/output actions that processes utiliz ewhich are available in a particular set.

%This may seems restrictive, but a large class of dist. systems are round-based....

%In the lifetime of dsitributed systems, processes are usually in subsets
%They're kind of moving in different hases, and even though technically you can be anywhere, the execution flow is somewhat...

\subsection{Decidability for Well-Behaved Guarded Processes}

Based on the notion of well-behavedness, we can now obtain a decidability 
result that works in the presence of guards. The following theorem implies 
that parameterized verification for properties $\phi_m(\ls)$ is decidable 
for well-behaved processes.

\begin{theorem}
\label{thm:GPS-with-guards}
If $\M_\infty$ is based on a well-behaved GSP process, then
$\M_\infty$ is a WSTS and we can effectively compute Pred.
\end{theorem}

\begin{proof}
To prove that $\M_\infty$ is a WSTS, we show compatibility of 
transitions w.r.t. $\altwqo$, i.e., 
if $\conf \altwqo \altconf$ and $\conf \rightarrow \conf'$, 
then $\exists \altconf'$ with $\conf' \altwqo \altconf'$ and $\altconf 
\rightarrow^* \altconf'$.
We consider three cases: (i) $k$-sender, (ii) $k$-maximal, and (iii) internal transitions.

(i) Suppose $a$ is a $k$-sender action. Let 
$\trans{\conf}{a, \guard}{\conf'}$ be a transition and $\conf \altwqo 
\altconf$.
Since $\conf \altwqo \altconf$ implies that $\supp(\altconf) \subseteq \guard$, we know that transition $\trans{\altconf}{a, \guard}{\altconf'}$ 
is possible, and by the proof of \thmref{generalizedBC} we know that 
$\conf' \wqo \altconf'$. To prove compatibility with respect to $\altwqo$, it 
remains to show that $\forall \guard' \in \guardset: (\supp(\conf')\subseteq 
\guard' \Rightarrow \supp(\altconf')\subseteq \guard')$.


First assume that condition~\eqref{eq:guard-comp-k-sender} holds. 
Then, let $\guard' \in \guardset$ be an arbitrary guard. By \eqref{eq:guard-comp-k-sender}, 
we either have $\senderset \not\subseteq \guard'$, in which case the 
desired condition is satisfied for $\guard'$, or we have that $\forall \ls \in
 \guard{:}~ M_a(\ls) \in \guard'$, i.e., all potential receivers move into $
\guard'$. Thus, we get $\supp(\conf')\subseteq \guard'$ iff $\supp(\altconf')
\subseteq \guard'$, satisfying the desired condition.

If instead of \eqref{eq:guard-comp-k-sender} the action satisfies \eqref{eq:guard-comp-k-sender-weak}, the argument is the same, except that if necessary we use the internal transitions \mn{removed: ``that are guaranteed to exist by the condition''}to arrive in a state $\altconf'$ with $\conf' \wqo \altconf'$.

(ii) Suppose $a$ is a $k$-maximal action with local transitions 
$\trans{\ls_i}{a_i!!,G}{\ls_i'}$ for $i \in \{1,\ldots,k\}$ and synchronization 
matrix $M_a$. By the proof of \thmref{generalizedBC} we know that there exists a transition $\trans{\altconf}{a, \guard}{\altconf'}$ with
$\conf' \wqo \altconf'$, and it remains to show that $\forall \guard' \in \guardset: (\supp(\conf')\subseteq 
\guard' \iff \supp(\altconf')\subseteq \guard')$. 

Let $\guard' \in \guardset$ be an arbitrary guard, and assume the action is strongly guard-compatible.
By condition \eqref{eq:guard-comp-k-max-1} we know that if there is a single 
local sending transition with $\ls_i' \in \guard'$, then all receivers will move into 
$\guard'$. 
So first suppose there is no such local transition: then $\guard'$ cannot be 
satisfied in $\conf'$ (since at least one sender must be present), and the 
desired property holds.
Inversely, suppose there is such a local transition: then all processes that start 
in $R$ will be mapped into $\guard'$, so $\guard'$ will be satisfied iff all 
remaining processes are mapped into $\guard'$.
Now, suppose that \emph{all} local transitions taken in 
$\trans{\conf}{a, \guard}{\conf'}$ are such that $\ls_i' \in \guard'$ 
(for otherwise $\conf'$ does not satisfy $\guard'$). 
Since $\conf \wqo \altconf$, there exists a transition $\trans{\altconf}{a, \guard}{\altconf'}$ such that the set of local 
transitions that are fired in $\trans{\conf}{a, \guard}{\conf'}$ is a 
subset of the local transitions that are fired in 
$\trans{\altconf}{a, \guard}{\altconf'}$. If all sending transitions 
taken in $\trans{\altconf}{a, \guard}{\altconf'}$ are also such that $\ls_i' 
\in \guard'$, then by conditions~\eqref{eq:guard-comp-k-max-1} and \eqref{eq:guard-comp-k-max-2} the same will hold for all receiving transitions from $\altconf$, and therefore, $\supp(\altconf') \subseteq \guard'$. Thus, 
suppose there is a local transition $\trans{\ls_i}{a_i!!,G}{\ls_i'}$ that is 
taken in $\trans{\altconf}{a, \guard}{\altconf'}$, but not in 
$\trans{\conf}{a, \guard}{\conf'}$, and $\ls_i' \notin \guard'$.
Let $\trans{\ls_j}{a_j!!,G}{\ls_j'}$ be an arbitrary local transition that is 
taken in $\trans{\conf}{a, \guard}{\conf'}$. Then by 
condition~\eqref{eq:guard-comp-k-max-2}, either there must be a guard 
$\guard'' \in \guardset'$ with $\ls_i \notin \guard'' \land \ls_j \in \guard''$, 
contradicting the assumption 
that $\conf \altwqo \altconf$, or we have $\ls_j' \in \guard' \Rightarrow \ls_i' \in 
\guard' \land M_a(\ls_i) \in \guard'$, contradicting the assumption that $\ls_
i' \notin \guard'$.

Again, if the action is weakly guard-compatible, the argument can be extended by using the paths of internal transitions \mn{removed ''guaranteed by the conditions''}, if necessary.

(iii) Suppose $a$ is an internal action with local transition $\trans{\ls}{a,G}{\ls'}$, let 
$\trans{\conf}{a, \guard}{\conf'}$ and $\conf \altwqo \altconf$.

%\swen{To support internal transitions and possibly some other cases, we need to have a form of non-strong compatibility that allows a transition to be ``repeated'' until a local state (or a set of states, for multiple senders) becomes empty. This may be necessary to finally arrive at a state that satisfies the same guards.}
If $\ls' \notin \guard'$ or $\ls \in \guard'$, we can simply take the same local transition from $\altconf$ and trivially, $\supp(\altconf') \subseteq \guard'$. If $\ls' \in \guard'$ and $\ls \notin \guard'$, then by condition~\eqref{eq:guard-comp-internal} every $t \in \guard$ has an executable path to a state $t'$ with $t' \triangleleft \ls'$, and therefore, by definition of $\triangleleft$, $t' \in \guard'$. For each of these states, if $\conf'(t)=0$ and $\altconf(t)>0$, then from $\altconf$ we take this path for all processes in $t$, and arrive in a state $\altconf'$ with $\conf' \altwqo \altconf'$.
%
%For $\guard \in \guardset$ and $\ls, t \in \LS$, write $\ls \leq_\guard t$ if $\ls \notin \guard$ implies $t \notin \guard$. Extended to the set of all guards, write $\ls \leq_\guardset t$ if there exists $\guard$ such that $\ls \leq_\guard t$.

The fact that we can effectively compute $Pred$ follows almost immediately 
from the proof of \thmref{generalizedBC}---the only difference is that we 
must take into account the guards, i.e., a predecessor is only valid if it 
additionally satisfies the guard of the transition under consideration.
\qed
\end{proof}


%\roopsha{Move to appendix}
%\para{The Environment Process in Broadcast Protocols.} \label{sec:gbc-env}
%While we do not consider an environment process in the \hlm, all of our results extend to the case with a distinguished process (or even multiple processes) that is not replicated. 
 %In fact, in the \hlm a system of the form $P_1 \ \| \ \ldots\ \| \ P_{n} \ \| \ E$ can be simulated by a system of the form $P_1' \ \| \ \ldots\ \| \ P_{n}' \ \| \ P_{n+1}'$ by letting $P'$ be a process that starts in an initial state where only a broadcast (on a fresh broadcast action) is possible, where the sender moves to the initial state of $E$ and all receivers move to the initial state of $P$. Moreover, the environment process is trivially well-behaved under the assumption that guards of regular processes do not depend on the state of the environment process, and that transitions of the environment process are not guarded.

%commented out since it is not needed for CAV submission
%\subsection{Well-behaved Broadcast Protocols with Global Conditions}
%\swen{looks like this whole subsection is not needed anymore, maybe except as inspiration for how to relax/generalize the third condition of well-behavedness}
%
%In this section, we show how some interesting classes of systems can be modeled as broadcast protocols with global conditions that are \emph{well-behaved}, i.e., satisfy condition~\eqref{cond:compatibility}. The first class supersedes several variants of our first example, the smoke detector, and the second class supersedes additional examples that we will present in Section~\ref{sec:evaluation}.
%
%In the following, we say that a transition of a process $P$ is \emph{\free} if it does not depend on other processes, i.e., it is an internal transition, a sending transition, or a negotiation \nour{The term negotiation was not defined before are we referring to consensus or?}\swen{it is introduced in 4.3, but we could make it more prominent}. It is \emph{$\guard$-\neutral} for $\guard \subseteq \LS$ if it does not require other processes that are in $\guard$ to change their state. A path from one state to another is \free (or $\guard$-\neutral) if all transitions on the path are \free (or $\guard$-\neutral). 
%
%\subsubsection{Round-based Systems}
%\label{sec:round-based}
%
%An interesting class of systems are those in which guarded transitions are used to synchronize all processes in regular intervals, ensuring that all processes agree on the ``round'' or ``phase'' the global system currently exhibits. Such systems can be modeled as broadcast protocols with global conditions under the following conditions:
%
%\begin{itemize}
%\item The local state space of the processes is partitioned \nour{does this imply disjointness?} into a sequence $\LS_1,\guard_1,\ldots,\LS_n,\guard_n \subseteq \LS$.
%\item Every transition from a state $\ls \in \LS_i$ either leads to $\LS_i$ or $\guard_i$.
%\item Every transition from a state $\ls \in \guard_i$ either leads to $\LS_i, \guard_i, \LS_{i+1}$ or $\guard_{i+1}$. If it leads to $\LS_{i+1}$ or $\guard_{i+1}$, then it is guarded with $\guard_i$. From $\guard_n$, transitions may lead to $\LS_1$ or $\guard_1$ under the same condition.
%\item From every global state $\conf$ where at least one process is in $\guard_i$ (i.e., with $\conf(\ls)>0$ for at least one $\ls \in \guard_i$), there is a $\guard_i$-\neutral path to a state $\conf'$ where all processes are in $\guard_i$ (i.e., with $\conf(\ls)=0$ for all $\ls \notin \guard_i$). \swen{this is stronger than before; it does not assume that there is a process in $\supp(\guard_i)$} 
%\end{itemize}
%
%One can easily show that if in such a system all processes start in some $\ls_0 \in \LS_1 \cup \guard_1$, then the processes will always agree on the current round, i.e., at every point in time there is an $i$ such that all processes are in $\LS_i \cup \guard_i$. Therefore, the last item implies condition~\eqref{cond:compatibility}. 
%
%While this definition reduces checking condition~\eqref{cond:compatibility} for the whole system to checking it for each round, the last item still requires an argument over global systems of parametric size. The following local condition implies the last item and can be used alternatively:
%
%\begin{itemize}
%\item For every $i \in \{1,\ldots,n\}$ and $\ls \in \LS_i$, there exists a \free and $\guard_i$-neutral path to a state in $\guard_i$. \swen{this is another strengthening; now local states need free and neutral paths to $G_i$ regardless of whether $G_i$ is already occupied}
%\end{itemize}
%
%Note that this condition is strictly stronger than the first one, i.e., it does not capture some systems that are captured by the first. However, since it is completely local it can be checked syntactically on the description of a single process.
%
%%Furthermore, note that one can easily find exceptions to the conditions above such that condition~\eqref{cond:compatibility} is still implied. For example, the $C_i$ do not need to be disjoint, as long as we have the following property: if $q$ appears in multiple $C_i$, then 
%
%\subsubsection{Systems with Layered Guards}
%
%A system is also well-behaved if it satisfies the following conditions, essentially modeling successively more restrictive access to ``deeper'' areas of the system:
%
%\begin{itemize}
%\item The local state space of processes is partitioned into $\bigcup_{i=1}^n \guard_i$ and $\overline{\guard}=\LS \setminus \bigcup_{i=1}^n \guard_i$, where $\guard_1 \subset \guard_2 \subset \ldots \subset \guard_n$.
%\item Transitions from $\overline{\guard}$ lead either to $\overline{\guard}$ or to $\guard_1$.
%\item For $1 \leq i \leq n$, transitions from $\guard_i$ lead either to $\guard_j$ with $j \geq i$, to $\overline{\guard}$, or to $\guard_1$. If the transition does not lead to $\guard_i$, then it is guarded with $\guard_i$.
%\item If there are transitions from $\overline{\guard}$ to $\guard_1$, then for $1 \leq i \leq n$ and every $\ls \in \guard_i$ there is a \free path to $\guard_1$ that is $\guard_j$-\neutral for $j < i$. \swen{not sure if this is what we want; reconsider!}
%\end{itemize}
%
%%\swen{need to add correctness argument?}
%
%%
%%\begin{lemma}
%%\label{lem:compatibility}
%%The WQO $\wqo$ defined above is compatible with a transition relation defined by broadcasts with global conditions if every transition $\trans{q}{a!!}{q'}$ with $q' \in C$ belongs to one of the following classes:\footnote{These conditions are generalizations of the ``flush'' and ``push'' transitions in \cite{emerson2003modela,emerson2003modelb}}
%%\begin{enumerate}
%%\item it is a \emph{$C$-flush}, i.e., for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, we have $p' \in C$;
%%\item it is a \emph{$\overline{C}$-flush}, i.e., for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, we have $p' \in \overline{C}$;
%%\item it is a \emph{$C$-neutral push transition}, i.e., there is a matching transition $\trans{q}{a??}{q}$, and for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, there is a self-loop $\trans{p'}{a??}{p'}$ and we have $p' \in C$ iff $p \in C$. In particular, it means that the broadcast matrix $M_a$ must be idempotent and map all elements to their own partition.\footnote{Note that this last condition covers the case of a single process making a local transition into $C$.}
%%\end{enumerate}
%%Note that the conditions need only hold if the guard of the transition is enabled, i.e., we do not care about matching transitions that can never be taken because of the guard of the initiating transition.
%%\end{lemma}
%%
%%\begin{proof}
%%As in \cite{EsparzaFM99}, it is sufficient to show compatibility for every action $a$ separately. Note that if $\conf \wqo \conf'$, then any \emph{guarded} transition will be enabled in $\conf$ iff it is enabled in $\conf'$, since by definition of $\wqo$ they have to agree on whether there are processes in $\overline{C}$. 
%%
%%First, consider a transition $\trans{q}{a!!}{q'}$ such that $q' \in \overline{C}$. Clearly, if $\conf \wqo \conf'$ and $\trans{\conf}{a}{\altconf}$, then for $\trans{\conf'}{a}{\altconf'}$ we have $\altconf \wqo \altconf'$, since $\overline{C}$ cannot be empty after any such transition, and $\altconf$ and $\altconf'$ agree on this.
%%
%%The most interesting case is when we have $\trans{q}{a!!}{q'}$ such that $q' \in C$: in this case, a ``disagreement'' between $\altconf$ and $\altconf'$ on whether there are processes in $\overline{C}$ happens in two cases: i) if $\conf(q)=1$, $\conf'(q)>1$, and $M_a(q) \in \overline{C}$, while all other states that appear in $\conf$ are mapped to $C$ by $M_a$, or ii) all states that appear in $\conf$ are mapped to $C$ by $M_a$, but there is a $p \in Q$ with $\conf(p)=0$, $\conf'(p)>0$ and $M_a(p) \in \overline{C}$. The conditions mentioned in the lemma deal with this problem in two different ways: the first two conditions ensure directly that $\altconf$ and $\altconf'$ agree on whether there are processes in $\overline{C}$, while the last condition ensures that there exists a sequence of transitions (all with the same action $a$) such that we have $\transcl{\altconf}{a}{\altconf''}$, where $\altconf$ and $\altconf''$ agree on whether there are processes in $\overline{C}$, and $\altconf \wqo \altconf'$. (\emph{Note:} if we allow guards on subsets of $C$, then we require the additional conditions whenever we ``leave'' one of these blocks)
%%\end{proof}
%%
%%We do not make a claim about the generality of these sufficient conditions. Instead, they should be seen as templates for similar conditions that allow to obtain decidability results for other types of systems with the same proof method. 
%%
%
%%\subsection{Additional Thoughts}
%%Questions to consider:
%%\begin{itemize}
%%\item Making transitions available if \textbf{all} processes are in a subset of the state space is similar to conjunctive guards in guarded protocols. Compare to decidability and undecidability results by Emerson and Kahlon~\cite{emerson2003model,emerson2003modela,emerson2003modelb}! They can model check LTL$\setminus$X properties for some models, can we also do that? (tree-saturation methods as in \cite{FS01} are not sufficient, but we could directly use the proof methods of EK...)
%%\item How can we include a counter for the case that we want \emph{at least $k$} processes to take some transition? (we might not have to - we could have $k$ ``layers'' in every local state space; then we only need to ``reset'' the processes in ``lose'' if everybody is in ``lose'' or ``win'')
%%\end{itemize}

==> PVprelims.tex <==
\section{Parameterized Correctness Arguments and Cutoffs}
\label{sec:parameterized}
\edit{
New sections structure:\\
1- keep 4.1: the basic model \\
2- merge 4.2 and 4.4: call this the extended model \\
3- introduce classes of well-behaved systems (current sec 4.5) \\
4- give cutoff arguments for those systems (current sec 4.6) \\
5- give the mapping section here (current sec 4.7)\\ 
6- conclude with a full example about the intro example (current sec 4.3): show a sketch of the mapping? which class of systems it falls under? cutoff argument?
7- parametric completion details and arguments.
}


In this section, we show how to obtain parameterized correctness arguments for our systems. To this end, we provide a model-checking procedure based on a counter representation, as well as a way to obtain cutoffs. We use a system model that is at a slightly higher level than the one in the previous sections, and is based on the model for broadcast protocols by \citet{EsparzaFM99}. After introducing this basic model, we extend it such that we can model the essential properties of \ch and certain kinds of transition guards. Then, we provide conditions for decidability of the PMCP of these systems, as well as a model-checking procedure and a way to derive cutoffs.

\subsection{Basic System Model: Broadcast Protocols} \label{basicModel}
We consider processes $P=\tuple{A,\LS,\ls_0,T}$, where $A$ is a finite set of action names that gives rise to the input actions $I = \{ a?? \mid a \in A \}$ and output actions $O = \{ a!! \mid a \in A\}$, $S$ is a finite set of states, $\ls_0 \in \LS$ is the initial state, and $T \subseteq \LS \times I \cup O \times S$ is the transition relation\footnote{In contrast to \secref{basicmodel}, we do not separate a state into a location and a valuation of variables in this model, and processes do not have identifiers.}. Without loss of generality, we assume that all actions are broadcasts, since this allows us to simulate local transitions, pairwise rendezvous and global synchronization. 
The semantics of broadcasts is: if some process takes a transition with $a!!$, then all other processes have to take a transition with $a??$ (if they have one in the current state; we can assume wlog that this is always the case, by adding self-loops). This part is exactly the model from Esparza et al.~\cite{EsparzaFM99}.

%Additionally, we assume that processes keep two counters $c_1$ and $c_2$ that range from $0$ to $n$, where $n$ is the number of processes in (this instance of) the system. Then, we distinguish three types of transitions:
%\begin{enumerate}
%\item regular broadcast transitions;
%\item \emph{counting transitions} that do not change the states of processes, but update all the counters. A counting transition is relative to a subset $Q_a \subset Q$, and after the transition, $c_1$ will be equal to the number of processes currently in $Q_a$, and $c_2$ will be equal to the number of processes in $Q \setminus Q_a$. We assume that the counters of all processes are updated in a uniform way, i.e., it is enough to keep each counter once; and
%\item \emph{majority transitions} that update the local states of all processes and reset the counters. Here, the update is similar to a broadcast update, except that any given majority transition is either only enabled if $c_1 \geq c_2$, or only if $c_1 < c_2$. 
%\end{enumerate}

Formally, the parameterized model of Esparza et al. is the following:
\begin{itemize}
	\item the state space of the parameterized system is $\GS = \Nats^{|\LS|}$, i.e., a state is a vector of natural numbers, representing the number of processes that are in any given state $\ls \in \LS$.
	%\footnote{Note that full symmetry of our systems, as shown in Lemma~\ref{}, is a precondition for this abstraction of the state space to be complete.}
	\item in a broadcast transition, one process makes a transition \trans{\ls_i}{a!!}{\ls_j} and all other processes make a transition \trans{\ls_k}{a??}{\ls_l}, depending on their current state $\ls_k$. Thus, the successor configuration $\conf' \in \Nats^{|\LS|}$ of a given configuration $\conf \in \Nats^{|\LS|}$ can be computed in the following way (where $\mathbf{u}_i$ is the unit vector with $\mathbf{u}_i(\ls_i)=1$):
	\[ \begin{array}{lll}
			\altconf 				& = & \conf - \mathbf{u}_i\\ 
			\altconf'(\ls_l) 	& = & \sum_{\{ \ls_k ~\mid~ \trans{\ls_k}{a??}{\ls_l} \}} \altconf(\ls_k)\\
			\conf' 						& = & \altconf' + \mathbf{u}_j.
		 \end{array}
		\]
		
%	while $c_1$ and $c_2$ remain unchanged.
		
	As noted by Esparza et al., the computation of $\conf'$ can be denoted more succinctly as $\conf' = M_a \cdot \conf + \mathbf{v}_a$, where $M_a$ is a \emph{broadcast matrix} that models the second line above and $\mathbf{v}_a$ is a \emph{broadcast vector} that models the effect of the other two lines. Under the assumption of deterministic transitions, in a broadcast matrix each column is a unit vector. 
	%\item in a counting transition, the configuration $\conf$ is unchanged, while $c_1$ and $c_2$ are updated according to a set $Q_a$:
	%\[ \begin{array}{lll}
			%c_1 & = & \sum_{\ls \in Q_a} \conf(\ls)\\ 
			%c_2	& = & \sum_{\ls \notin Q_a} \conf(\ls).
		 %\end{array}
		%\]
		%
	%We assume that counting transitions are only enabled when all processes are in a fixed subset $Q_c$ of the state space $Q$, and then they have to be taken.
	%\item for a majority transition, the successor configuration is defined by $\conf' = M \cdot \conf + \mathbf{v}$, $c_1' = c_2' =0$, and there are two possible choices for $M$ and $\mathbf{v}$: if $c_1 \geq c_2$, then $\conf' = M_1 \cdot \conf + \mathbf{v}_1$, and otherwise $\conf' = M_2 \cdot \conf + \mathbf{v}_2$. We assume that majority transitions are only enabled when $c_1 \neq 0$ or $c_2 \neq 0$, and then they have to be taken. Note that this implies that a counting transition is always directly followed by a majority transition.
\end{itemize}

Broadcasts can be used to model the effect of \ch on a slightly more abstract level, where a single broadcast corresponds to $\ch(1)$, and $\ch(k)$ for $k \in \Nats$ can be modeled by a sequence of $k$ broadcasts. Since processes do not have identifiers and the model only keeps track of \emph{how many} processes are in each local state, this captures the effects of executing \ch as faithfully as possible. However, execution of \ch also has a precondition: all processes should be informed about all other processes, and should agree on who participates in \ch. This will be modeled by global conditions that allow us to constrain the system such that some transitions are only enabled in certain global states.
	
\subsection{Extended Model: Broadcasts with Global Conditions} \label{sec:extendedmodel}
We extend our model by considering transitions that can be guarded by a set of local states $\guard \subseteq \LS$, intuitively stating that the transition can only be taken if all processes are in $\guard$.

Formally, our systems are now given by $\tuple{A,\LS,\ls_0,T}$, where all components are as before, except that now we have $T \subseteq \LS \times I \cup O \times \guards \times \LS$. The update of global state $\conf$ by a transition is defined as before, but a transition is only enabled if $\conf$ satisfies the guard $\guard$, i.e., if $\conf(\ls)=0$ for all $\ls \notin \guard$.

\subsection{The Smoke Detector Example in this Model}

%\resizebox{\textwidth}{!}{\includegraphics{example.png}}
\input{smokemodel}
To clarify the relation to the previous model, let us consider again the smoke detector in~\figref{introExample}. First, note that the transition from $Env$ to $Init$ sets a local variable. Since in this model we do not keep track of local variables, this means we have to split into two different states. Then, note that states $Init$, $Wait$ and $Store$ are used to synchronize all processes, i.e., every process can only leave $Wait$ into $Idle$ or $Pick$ if it has heard from all other processes. For parameterized verification, we summarize the synchronization of process into a single negotiation step, i.e., a broadcast that does not have a dedicated sender, but all nodes simultaneously take a transition according to their current local state\footnote{Systems that only communicate through negotiation have been investigated by \citet{ED13}.}: from $Wait_2$, the process moves to $Pick$, and from $Wait_1$ to $Idle$. To ensure that this can only happen if all processes are ready, we add a guard that requires all processes to be in either $Wait_1$ or $Wait_2$ for this transition to be enabled. Then, the \ch(2) can be modeled by a sequence of two broadcast transitions, which we summarize in a single transition that takes $2$ processes to $Rep.$ and all other processes that are in $Pick$ to $Idle$, as shown in~\figref{smoke-sensors-param}.



%We have a chain of $k$ broadcasts on action ``choose'', to ensure that exactly $k$ processes can move to ``win''. For the case where less than $k$ processes are available for ``choose'', consider a system with the following changes:
%\begin{itemize}
%\item state ``win'' is a part of $C$, i.e., $C=\{c_1,c_2,win\}$
%\item all states where a choose transition is possible have additional transitions to the initial state, which are guarded with $\forall C$. When these transitions to the initial state are taken, the process has to remember how many choose actions it has already taken and enter the line of choose operations in the right place when the next ``done'' is taken.
%\end{itemize}
%
%\nour{why are we adding this last point? are we supporting a system where < k win and the rest are still in detect, trying to enter the critical section with whatever remaining capacity? e.g.  capacity = 5, 2 enter win, the rest of processes fight over the 3 spots?}
%\roopsha{Perhaps add this as a note that it could be done?}


==> WSTS.tex <==
\subsection{Model Checking for Broadcast Protocols with Global Conditions} \label{parametrizedSafety}

\citet{Finkel87} introduced the notion of a well-structured transition system (WSTS): an infinite-state transition system that is equipped with a \emph{well-quasi order (WQO)} on its state space and that has some additional properties. We will use \citet{FS01} as a main reference, which gives a survey of existing results and puts them into a common framework. In particular, these results show how we can effectively represent systems with infinite sets of states in order to decide safety/reachability properties.

In this section we show that, under some additional conditions, broadcast protocols with global conditions are WSTSs, and we can decide the parameterized model checking problem (PMCP) for safety properties. 

%\subsection{The Well-Quasi Order}
%
%Given the set $C \subset Q$ that defines the partition of local states, we define the WQO on global states as 
%$$\conf \wqo \conf' \text{ iff } \left(\conf(q) \leq \conf'(q) \text{ for all } q \in Q \text{ and } \sum_{q \notin C}\conf(q)=0 \text{ iff } \sum_{q \notin C}\conf(q)=0\right).$$
%
%That is, $\conf'$ must contain at least as many processes as $\conf$ in every local state, and the two configurations must agree on whether all processes are in $C$.

\closeparagraph{Compatibility and Effective Computability of Predecessors}
%
To prove decidability of the PMCP, we need some additional definitions.

\begin{definition}
A WQO $\wqo$ is \emph{compatible} with a transition relation $\rightarrow$ if for every $\conf \wqo \conf'$ and $\conf \rightarrow \altconf$ there exists $\altconf'$ with $\altconf \wqo \altconf'$ and $\conf' \rightarrow^* \altconf'$.
\end{definition}

A transition system equipped with a WQO that is compatible with its transition relation is called a \emph{well-structured transition system (WSTS)}.

Fix an infinite set of states $\GS$ and a transition relation $\rightarrow$. For a (possibly infinite) subset $U \subseteq \GS$, let $Pred(U)$ denote the predecessor states of $U$ with respect to $\rightarrow$. Furthermore, let $\uparrow U$ denote the \emph{upwards closure} of $U$, i.e., the set of all states $\altconf$ such that there exists $\conf \in U$ with $\conf \wqo \altconf$. A set $U$ is upwards closed if $\uparrow U = U$. Every upwards closed set $U$ has a finite \emph{basis}: a finite set $B \subseteq U$ such that $\uparrow B = U$. %We also denote the basis of $U$ by $basis(U)$.

\begin{definition}
For a given transition relation $\rightarrow$ and WQO $\wqo$, we say that we can \emph{effectively compute $Pred$} if there exists an algorithm that computes a finite basis of $Pred(U)$ from any finite basis of any upwards-closed $U \subseteq \GS$. 
\end{definition}

\citet{FS01} have shown that we can decide reachability of any upwards-closed set in a WSTS if we can effectively compute $Pred$.

\closeparagraph{Deciding Safety Properties for Broadcast Protocols with Global Conditions.}
%
\citet{EsparzaFM99} have defined the following WQO on the (global) states of the basic model of broadcast protocols:

$$\conf \wqo \conf' \text{ iff }\conf(\ls) \leq \conf'(\ls) \text{ for all } \ls \in \LS.$$

%, and one of the following holds:
%\begin{enumerate}
%\item $c_1=c_2=c_1'=c_2'=0$ and $\sum_{q \notin Q_c} \conf(q) > 0 < \sum_{q \notin Q_c} \conf'(q)$, 
%\item $c_1=c_2=c_1'=c_2'=0$ and $\sum_{q \notin Q_c} \conf(q) = 0 = \sum_{q \notin Q_c} \conf'(q)$,
%\item $c_1>0<c_1'$, $c_1 \geq c_2$ and $c_1' \geq c_2'$, or
%\item $c_2>0<c_2'$, $c_1 < c_2$ and $c_1' < c_2'$.
%\end{enumerate}
%Note that the well quasi order is only partially defined, and it is undefined for almost all pairs of states in instances of the same size: $\conf(q) \leq \conf'(q)$ for all $q \in Q$ can only hold if the instance of $\conf'$ is at least as big as the instance of $\conf$, and if their size is equal it can only hold if $\conf(q)=\conf'(q)$ for all $q$.

Based on this, they have shown:
\begin{theorem}[\cite{EsparzaFM99}]
\label{thm:compatibility}
For the model of broadcast protocols and the WQO above, the following hold:
\begin{itemize}
\item Broadcast transitions are \emph{strongly compatible} with the WQO, i.e., if $\conf \wqo \conf'$ and $\conf \rightarrow \altconf$, then $\exists \altconf'$ with $\altconf \wqo \altconf'$ and $\conf' \rightarrow \altconf'$. This implies that for a given upward-closed set of states $C$, the set of predecessor states $Pred(C)$ is also upward-closed.\footnote{In fact, Esparza et al. have only proven the latter, but one can show that the two statements are equivalent.}
\item For broadcast transition systems we can effectively compute Pred. 
\end{itemize}
\end{theorem}

We quickly recapitulate their proof idea, because it will inform our proofs for broadcast protocols with global conditions.

\begin{proof}
For both items, it is sufficient to show them for every action $a \in A$ separately. With our formulation, the first item is easy to show based on the matrix notation of broadcast transitions. For the second, observe that for a transition based on $\trans{\ls_k}{a!!}{\ls_l}$, any element $\conf$ of $Pred(C)$ must satisfy $\conf(\ls_k) \geq 1$ and $M_a \cdot \conf + \mathbf{v}_a = \conf'$, for some $\conf' \in C$. The basis of $Pred(C)$ consists of the minimal elements that satisfy these conditions, and thus is computable.
\end{proof}


In the following, we consider the extended model of broadcast protocols with global conditions and show under which conditions we can obtain a similar result. 
For a guard $G \subseteq \LS$, let $\supp(G)\subseteq \LS$ be the set of local states from which there is a transition guarded by $G$. We call this set the \emph{support} of $G$.

\begin{lemma}
\label{lem:compatibility}
A broadcast system with global conditions based on a set of guards $\{ \guard_1,\ldots,\guard_n\}$ and with the WQO $\wqo$ is a WSTS with effectively computable Pred iff the following condition holds:
\begin{equation}
\tag{$*$}
\begin{minipage}{.9\textwidth}
For every $\conf \in \GS$ and every $\guard_i$ s.t. $\exists \ls \in \supp(\guard_i): \conf(\ls)>0$ and $\exists \ls \notin \guard_i: \conf(\ls)>0$, there exists a path from $\conf$ to a state $\altconf$ with $\altconf(\ls)=0$ for all $\ls \notin \guard_i$, and $\altconf(\ls) \geq \conf(\ls)$ for all $\ls \in \guard_i$.
\end{minipage}
\label{cond:compatibility}
\end{equation}
\end{lemma}

\swen{proof needs to be reconsidered; in particular, it needs to go both directions}


\begin{proof}
To see that the transition relation $\rightarrow$ is compatible with $\wqo$, first note that, as for broadcast protocols without global conditions, we can look at every action $a \in A$ separately. Then, for transitions $\trans{\ls_k}{a!!}{\ls_l}$ without guards, the same argument as in the original proof holds. Finally, consider a transition $\trans{\ls_k}{a!!}{\ls_l}$ with a guard $\guard_i$: to ensure compatibility, if $\conf \wqo \conf'$ and $\trans{\conf}{a}{\altconf}$, then there must exist a sequence of transitions $\transcl{\conf'}{\altconf'}$ with $\altconf \wqo \altconf'$. Note that condition~\eqref{cond:compatibility} ensures that from $\conf'$ we can reach a state $\conf''$ (with $\conf''(\ls)=0$ for all $\ls \notin \guard_i$) in which the guard is enabled, and with $\conf \wqo \conf''$. Thus, we can take transition $\trans{\conf''}{a}{\altconf'}$, where we know that $\altconf \wqo \altconf'$ by the first item of Theorem~\ref{thm:compatibility}.

\begin{center}
\begin{tikzpicture}[node distance=5em]
\node (conf) {$\conf$};

\node[below of=conf] (conf') {$\conf'$};

\node[right of=conf'] (conf'') {$\conf''$};

\node[right of=conf''] (altconf') {$\altconf'$};

\node[above of=altconf'] (altconf) {$\altconf$};

\path[->] (conf) edge node[above]{$a$} (altconf);

\path[->] (conf) edge node[right]{$\wqo$} (conf');

\path[->] (conf') edge node[above]{\eqref{cond:compatibility}} (conf'');

\path[->] (conf'') edge node[above]{$a$} (altconf');

\path[->] (altconf) edge node[right]{$\wqo$} (altconf');

 %@>\phantom{phantom text}a\phantom{phantom text}>> @. \conf'\\
%@VV\wqo V	@.	@VV\wqo V\\
%\altconf @>\eqref{cond:compatibility}>> \altconf'' @>a>> \altconf'\\
%\end{CD}
\end{tikzpicture}
\end{center}
%\nour{Notation suggestion: in theorem 4.3 we used $q \rightarrow p$ in the smaller system and $q' \rightarrow p'$ in the bigger system. Here we used  $q \rightarrow q'$ in the smaller system and $p \rightarrow p'$ in the bigger system. It would probably read nicer if we unify them.}
To see that we have effectively computable $Pred$, again note that we can consider transitions separately, and the interesting case are transitions with a guard. For these, we can compute the basis of their predecessor states in the same way as for transitions without guards, and then remove states $\conf$ that do not satisfy the guard. This is sound since if $\conf$ does not satisfy the guard, then no state in $\uparrow \conf$ can satisfy the guard.

\swen{it is not a necessary condition right now; for this we need an additional assumption that guarded transitions can not be replaced by (a sequence of) unguarded transitions; this seems to hold for round-based systems and systems with layered guards}
\end{proof}

From Lemma~\ref{lem:compatibility} and \citet[Theorem 3.6]{FS01}, we obtain:

\begin{theorem}
\label{thm:decidability}
Let $(\GS,\rightarrow)$ be a broadcast protocol with global conditions that satisfies condition~\eqref{cond:compatibility} and $U \subseteq \GS$ an upwards-closed set of states. Then we can decide whether states in $U$ are reachable.
\end{theorem}

Similar to \cite{EsparzaFM99}, this extends to general safety properties by considering a system that runs the broadcast protocol in parallel to a safety automaton for the desired property.

%Similar to the results of \citet{EsparzaFM99}, this extends to general safety properties by considering a system that runs the broadcast protocol in parallel to a safety automaton for the desired property.


\subsection{Well-behaved Broadcast Protocols with Global Conditions}

In this section, we show how some interesting classes of systems can be modeled as broadcast protocols with global conditions that are \emph{well-behaved}, i.e., satisfy condition~\eqref{cond:compatibility}. The first class supersedes several variants of our first example, the smoke detector, and the second class supersedes additional examples that we will present in Section~\ref{sec:evaluation}.

In the following, we say that a transition of a process $P$ is \emph{\free} if it does not depend on other processes, i.e., it is an internal transition, a sending transition, or a negotiation \nour{The term negotiation was not defined before are we referring to consensus or?}\swen{it is introduced in 4.3, but we could make it more prominent}. It is \emph{$\guard$-\neutral} for $\guard \subseteq \LS$ if it does not require other processes that are in $\guard$ to change their state. A path from one state to another is \free (or $\guard$-\neutral) if all transitions on the path are \free (or $\guard$-\neutral). 

\subsubsection{Round-based Systems}
\label{sec:round-based}

An interesting class of systems are those in which guarded transitions are used to synchronize all processes in regular intervals, ensuring that all processes agree on the ``round'' or ``phase'' the global system currently exhibits. Such systems can be modeled as broadcast protocols with global conditions under the following conditions:

\begin{itemize}
\item The local state space of the processes is partitioned \nour{does this imply disjointness?} into a sequence $\LS_1,\guard_1,\ldots,\LS_n,\guard_n \subseteq \LS$.
\item Every transition from a state $\ls \in \LS_i$ either leads to $\LS_i$ or $\guard_i$.
\item Every transition from a state $\ls \in \guard_i$ either leads to $\LS_i, \guard_i, \LS_{i+1}$ or $\guard_{i+1}$. If it leads to $\LS_{i+1}$ or $\guard_{i+1}$, then it is guarded with $\guard_i$. From $\guard_n$, transitions may lead to $\LS_1$ or $\guard_1$ under the same condition.
\item From every global state $\conf$ where at least one process is in $\guard_i$ (i.e., with $\conf(\ls)>0$ for at least one $\ls \in \guard_i$), there is a $\guard_i$-\neutral path to a state $\conf'$ where all processes are in $\guard_i$ (i.e., with $\conf(\ls)=0$ for all $\ls \notin \guard_i$). \swen{this is stronger than before; it does not assume that there is a process in $\supp(\guard_i)$} 
\end{itemize}

One can easily show that if in such a system all processes start in some $\ls_0 \in \LS_1 \cup \guard_1$, then the processes will always agree on the current round, i.e., at every point in time there is an $i$ such that all processes are in $\LS_i \cup \guard_i$. Therefore, the last item implies condition~\eqref{cond:compatibility}. 

While this definition reduces checking condition~\eqref{cond:compatibility} for the whole system to checking it for each round, the last item still requires an argument over global systems of parametric size. The following local condition implies the last item and can be used alternatively:

\begin{itemize}
\item For every $i \in \{1,\ldots,n\}$ and $\ls \in \LS_i$, there exists a \free and $\guard_i$-neutral path to a state in $\guard_i$. \swen{this is another strengthening; now local states need free and neutral paths to $G_i$ regardless of whether $G_i$ is already occupied}
\end{itemize}

Note that this condition is strictly stronger than the first one, i.e., it does not capture some systems that are captured by the first. However, since it is completely local it can be checked syntactically on the description of a single process.

%Furthermore, note that one can easily find exceptions to the conditions above such that condition~\eqref{cond:compatibility} is still implied. For example, the $C_i$ do not need to be disjoint, as long as we have the following property: if $q$ appears in multiple $C_i$, then 

\subsubsection{Systems with Layered Guards}

A system is also well-behaved if it satisfies the following conditions, essentially modeling successively more restrictive access to ``deeper'' areas of the system:

\begin{itemize}
\item The local state space of processes is partitioned into $\bigcup_{i=1}^n \guard_i$ and $\overline{\guard}=\LS \setminus \bigcup_{i=1}^n \guard_i$, where $\guard_1 \subset \guard_2 \subset \ldots \subset \guard_n$.
\item Transitions from $\overline{\guard}$ lead either to $\overline{\guard}$ or to $\guard_1$.
\item For $1 \leq i \leq n$, transitions from $\guard_i$ lead either to $\guard_j$ with $j \geq i$, to $\overline{\guard}$, or to $\guard_1$. If the transition does not lead to $\guard_i$, then it is guarded with $\guard_i$.
\item If there are transitions from $\overline{\guard}$ to $\guard_1$, then for $1 \leq i \leq n$ and every $\ls \in \guard_i$ there is a \free path to $\guard_1$ that is $\guard_j$-\neutral for $j < i$. \swen{not sure if this is what we want; reconsider!}
\end{itemize}

%\swen{need to add correctness argument?}

%
%\begin{lemma}
%\label{lem:compatibility}
%The WQO $\wqo$ defined above is compatible with a transition relation defined by broadcasts with global conditions if every transition $\trans{q}{a!!}{q'}$ with $q' \in C$ belongs to one of the following classes:\footnote{These conditions are generalizations of the ``flush'' and ``push'' transitions in \cite{emerson2003modela,emerson2003modelb}}
%\begin{enumerate}
%\item it is a \emph{$C$-flush}, i.e., for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, we have $p' \in C$;
%\item it is a \emph{$\overline{C}$-flush}, i.e., for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, we have $p' \in \overline{C}$;
%\item it is a \emph{$C$-neutral push transition}, i.e., there is a matching transition $\trans{q}{a??}{q}$, and for all $p \in Q$ and matching transitions $\trans{p}{a??}{p'}$, there is a self-loop $\trans{p'}{a??}{p'}$ and we have $p' \in C$ iff $p \in C$. In particular, it means that the broadcast matrix $M_a$ must be idempotent and map all elements to their own partition.\footnote{Note that this last condition covers the case of a single process making a local transition into $C$.}
%\end{enumerate}
%Note that the conditions need only hold if the guard of the transition is enabled, i.e., we do not care about matching transitions that can never be taken because of the guard of the initiating transition.
%\end{lemma}
%
%\begin{proof}
%As in \cite{EsparzaFM99}, it is sufficient to show compatibility for every action $a$ separately. Note that if $\conf \wqo \conf'$, then any \emph{guarded} transition will be enabled in $\conf$ iff it is enabled in $\conf'$, since by definition of $\wqo$ they have to agree on whether there are processes in $\overline{C}$. 
%
%First, consider a transition $\trans{q}{a!!}{q'}$ such that $q' \in \overline{C}$. Clearly, if $\conf \wqo \conf'$ and $\trans{\conf}{a}{\altconf}$, then for $\trans{\conf'}{a}{\altconf'}$ we have $\altconf \wqo \altconf'$, since $\overline{C}$ cannot be empty after any such transition, and $\altconf$ and $\altconf'$ agree on this.
%
%The most interesting case is when we have $\trans{q}{a!!}{q'}$ such that $q' \in C$: in this case, a ``disagreement'' between $\altconf$ and $\altconf'$ on whether there are processes in $\overline{C}$ happens in two cases: i) if $\conf(q)=1$, $\conf'(q)>1$, and $M_a(q) \in \overline{C}$, while all other states that appear in $\conf$ are mapped to $C$ by $M_a$, or ii) all states that appear in $\conf$ are mapped to $C$ by $M_a$, but there is a $p \in Q$ with $\conf(p)=0$, $\conf'(p)>0$ and $M_a(p) \in \overline{C}$. The conditions mentioned in the lemma deal with this problem in two different ways: the first two conditions ensure directly that $\altconf$ and $\altconf'$ agree on whether there are processes in $\overline{C}$, while the last condition ensures that there exists a sequence of transitions (all with the same action $a$) such that we have $\transcl{\altconf}{a}{\altconf''}$, where $\altconf$ and $\altconf''$ agree on whether there are processes in $\overline{C}$, and $\altconf \wqo \altconf'$. (\emph{Note:} if we allow guards on subsets of $C$, then we require the additional conditions whenever we ``leave'' one of these blocks)
%\end{proof}
%
%We do not make a claim about the generality of these sufficient conditions. Instead, they should be seen as templates for similar conditions that allow to obtain decidability results for other types of systems with the same proof method. 
%

%\subsection{Additional Thoughts}
%Questions to consider:
%\begin{itemize}
%\item Making transitions available if \textbf{all} processes are in a subset of the state space is similar to conjunctive guards in guarded protocols. Compare to decidability and undecidability results by Emerson and Kahlon~\cite{emerson2003model,emerson2003modela,emerson2003modelb}! They can model check LTL$\setminus$X properties for some models, can we also do that? (tree-saturation methods as in \cite{FS01} are not sufficient, but we could directly use the proof methods of EK...)
%\item How can we include a counter for the case that we want \emph{at least $k$} processes to take some transition? (we might not have to - we could have $k$ ``layers'' in every local state space; then we only need to ``reset'' the processes in ``lose'' if everybody is in ``lose'' or ``win'')
%\end{itemize}

==> cutoffExample.tex <==
\begin{example}
\chris{Are paths like $\st{\Env} \xrightarrow{\trr{\Smoke??}} \st{\Idle} \xrightarrow{\trr{\Resett}} \st{\Env} \rightarrow \st{\Ask} \xrightarrow{...} \st{\Pick} \xrightarrow{...} \st{\Report}$ considered? if so, lemma2 doesn't hold.\\ }
In this example we show how \lemref{cutoffnoreset} applies to the example in \figref{MappedIntroExample}. Here $\ls_0$ is the \st{\Env} state, $\ls$ is the \st{\Report} state, and the value of $m$ is 3 (since the safety specification is: no more than 2 detectors can report the fire). Consider the action \tr{Choose} to be a maximal-sender action.

The set of all paths from $\ls_0$ to $\ls$ is:
\begin{compactenum}[--]
\item $\st{\Env} \xrightarrow{} \st{\Ask} \xrightarrow{\trr{\Smoke}!!} \st{\Pick} \xrightarrow{\trr{\Choose_1}!!} \st{\Report}$,
\item $\st{\Env} \xrightarrow{} \st{\Ask} \xrightarrow{\trr{\Smoke}!!} \st{\Pick} \xrightarrow{\trr{\Choose_2}!!} \st{\Report}$,
\item $\st{\Env} \xrightarrow{} \st{\Ask} \xrightarrow{\trr{\Smoke}??} \st{\Pick} \xrightarrow{\trr{\Choose_1}!!} \st{\Report}$, and,
\item $\st{\Env} \xrightarrow{} \st{\Ask} \xrightarrow{\trr{\Smoke}??} \st{\Pick} \xrightarrow{\trr{\Choose_2}!!} \st{\Report}$.
\end{compactenum}

It is clear that all transitions of those paths are free, according to our definitions. \nour{commented out details.}%since they are either sending transitions of maximal-sender action $\trr{\Choose_1}$ and $\trr{\Choose_1}$, the sending transition of 1-sender action \tr{\Smoke!!}, a broadcast-receive action with its corresponding sender \tr{\Smoke??}, or internal transitions.

Since \lemref{cutoffnoreset} holds, then reachability of $\ls$ is \nice and the cutoff is 3. 

\end{example}


%
%
%
%\begin{example}
%In this example we show how \lemref{cutoffnoreset} applies to the example in \figref{MappedIntroExample}. Here $\ls_0$ is the \st{\Env} state, $\ls$ is the \st{\Report} state, and the value of $m$ is 3 (since the safety specification is: no more than 2 detectors can report the fire).
%
%The set of simple paths $\mathcal{F}$ is:
%\begin{compactenum}[--]
%\item $\st{Env} \xrightarrow{} \st{Ask} \xrightarrow{\trr{\Smoke}!!} \st{Pick} \xrightarrow{\trr{\Choose_1}!!} \st{Report}$,
%\item $\st{Env} \xrightarrow{} \st{Ask} \xrightarrow{\trr{\Smoke}!!} \st{Pick} \xrightarrow{\trr{\Choose_2}!!} \st{Report}$,
%\item $\st{Env} \xrightarrow{} \st{Ask} \xrightarrow{\trr{\Smoke}??} \st{Pick} \xrightarrow{\trr{\Choose_1}!!} \st{Report}$, and,
%\item $\st{Env} \xrightarrow{} \st{Ask} \xrightarrow{\trr{\Smoke}??} \st{Pick} \xrightarrow{\trr{\Choose_2}!!} \st{Report}$.
%\end{compactenum}
%
%It is clear that all the sending transitions {$\trr{\Smoke}!!,\trr{\Choose_1}!!,\trr{\Choose_2}!!$} appear only in $\mathcal{F}$. Furthermore, along those paths, we have the following broadcast-receive transitions:
%\begin{compactenum}[--]
%\item the transition $\trans{\st{Env}}{\trr{\Smoke}??}{\st{Idle}}$ which is discarded because the internal transition $\trans{\st{Env}}{}{\st{Ask}}$ exists in a path in $\mathcal{F}$.
%\item the transition $\trans{\st{Ask}}{\trr{\Smoke}??}{\st{Pick}}$ leads to back to a state (\st{Pick}) to a path in $\mathcal{F}$ 
%\end{compactenum}
%
%Since \lemref{newcutoffLemma22} holds, then reachability of $\ls$ is \nice and the cutoff is 3. 
%
%\end{example}



==> cutoffsprocedure.tex <==
\renewcommand{\Comment}[2][.2\linewidth]{%
\leavevmode\hfill\makebox[#1][l]{$\rhd$~#2}}

\algnewcommand{\orr}{\textbf{ or }}
\begin{algorithm}
  \SetKwFunction{mapproc}{Cutoff}
  \SetKwProg{myproc}{procedure}{}{}
  \myproc{\mapproc{$\ph, \phi$}}{
  \SetKwInOut{Input}{Input}
  \SetKwInOut{Output}{Output}
  \Input{
  $\ph$, \wellbehaved process definition in the \hlm\\
  $\phi$, \permissible safety specification\\
  }
  \Output{$c$, a cutoff for $\ph$ and $\phi$, or \texttt{null}}
  \BlankLine

$m =$ \Call{NumberProcesses}{$\phi$}\\
$\mathcal{P}=${\Call{SimplePathsTo}{$\phi$}}\\
$\mathcal{F}=${\Call{SimpleFreePathsTo}{$\phi$}}\\
\If( \Comment{\lemref{newcutoffLemma22}}) {  \Call{ActionTypes}{$\ph$} $\subseteq Internal \cup Negotiation$     	\Comment{\lemref{cutoffnegotiation}}	\\  
\orr \Call{AllPathsTo}{$\phi$} $\subseteq$ \Call{FreePaths}{$\ph$} 		\Comment{\lemref{cutoffnoreset}}		\\
\orr $\mathcal{P} \subseteq$ \Call{FreePaths}{$\ph$} \textrm{\bf{and}} \Call{BCReceivesSatisfied}{$\ph, \mathcal{P}$} \Comment{\lemref{newcutoffLemma}} \\
\orr \Call{BCTransitionsSatisfied}{$\ph,\mathcal{F}$}}{  
\Return $m$
}

\Return {\texttt{null}}
}%
%mappable
  %$\ph = $ \Call{EncodeVariablesAndGuardedCommands}{$\ph$}  \label{line:states}\\
  %$\ph = $ \Call{GenerateGuardsForBroadcasts}{$\ph$}  \label{line:broadcast}\\
  %$\ph = $ \Call{RewriteChooseTransitions}{$\ph$}  \label{line:choose}\\
  %\Return $\ph$
%}
%\Else{
%\Return \tt{null}
%}
%%$\ph = \pl$ \\
%%$b =$ \Call{DetectBroadcastandCollect}{$\ph$} \label{line:chkbac}\\
%%\If {$b$}{
  %$\ph = $ \Call{RewriteBroadcastandCollect}{$\pl$} \label{line:rwbac}\\
%%}
%$mappable =$ \Call{Mappable}{$\ph$}\\
\caption{Procedure that determines cutoff for process $\ph$ and safety specification $\phi$}
\label{algo:cutoff}
\end{algorithm}

==> intro-sats-fig.tex <==
\begin{figure*}
\begin{minipage}{0.45\textwidth}
\begin{dsl}
  machine SATS {
  variables {
     bool direction
     Set set1 = N, set2, set3, set4, set5, 
         winners3, winners4, winners5 
  }     
  actions {
    env Miss : unit
    env Land : unit
    WhosInBase : unit
    Reply : {yes, no} 
  }
  initial state Fly {
    on [set2 , _] = Consensus(set1,5) do {
      if(set2.contains(self)) {
        goto Enter
      }
    } 
  }
  state Enter {
    on [set3 , set4] = Consensus(set2, 2) do {
      if(set3.contains(self)) {
        direction = left
        goto HoldLeft
      } else {
        direction = right
        goto HoldRight
      }
    } 
  }
  state HoldLeft {
    on [winners3 , _] = Consensus(set3, 1) do {
      if(winners3.contains(self)) {
        goto Base
      } else {
        goto Idle
      }
    } 
  }
  state HoldRight {
    on [winners4 , _] = Consensus(set4, 1) do {
      if(winners4.contains(self)) {
        Broadcast(WhosInBase)
        goto Base
      } else {
        goto Idle
      }
    } 
  }
\end{dsl}
\end{minipage}
\hfill
\begin{minipage}{0.45\textwidth}
\begin{dsl}
  state Base {
    on WhosInBase do {
      Send(Reply[yes], WhosInBase.sID)
    }
    on Reply do {
       if(Reply.value == yes) {
        set5.add(Reply.sID)
       }
        totalReplies++
      if(totalReplies == n-1) {
         goto Pick
      }
    }  
  }
  state Pick {
    on [winners , _] = Consensus(set5, 1) do {
      if(winners.contains(self)) {
        goto FinalApproach
      } else {
        goto Idle
      } 
    } 
  }
  state FinalApproach {
    on Miss do {
      if(direction = left) {
        goto HoldLeft
      } else {
        goto HoldRight
      }
    }
    on Land do {
      goto Runway
    } 
  }   
  state Idle {
    on WhosInBase do {
      Send(Reply[no], WhosInBase.sID)
    }
  }
}

\end{dsl}
\captionof{figure}{SATS DSL description\label{fig:satscode}} 


\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=5.1cm,semithick,scale=0.4,every node/.style={transform shape}]


\tikzstyle{every state}=[font=\fontsize{13}{0}\selectfont, thick, fill=white,align=center]
\tikzstyle{every edge}=[font=\fontsize{13}{0}\selectfont, draw = black]
%%% node (states) definition%%%%%%


  \node[state,minimum size=2cm]	(fly)										                  {\st{Fly}};
  \node[state,minimum size=2cm]	(enter)		[ right of=fly]					        {\st{Enter}};
  \node[state,minimum size=2cm]	(hold left)	[above right of=enter]		    {\st{Hold}\\\st{Left}};
  \node[state,minimum size=2cm] 	(hold right)	[below right of=enter] 		{\st{Hold}\\\st{Right}};
  \node[state,minimum size=2cm]	(base) 		[below right of=hold left] 		  {\st{Base}};
  \node[state,minimum size=2cm]	(final app) 	[right of=base]       			{\st{Final}\\\st{App}};
  %\node[state,minimum size=2cm]	(miss left) 	[above left of=final app]		{\st{Miss}\\\st{Left}};
  %\node[state,minimum size=2cm]	(miss right) 	[below left of=final app]   {\st{Miss}\\\st{Right}};
  \node[state,minimum size=2cm]	(runway) 	[below = 3.5 cm of final app]   	{\st{Runway}};
  %\node[state,minimum size=2cm]	(land) 		[left  of=runway]       			  {\st{Land}};


%%% paths definition%%%%%%


\draw
(fly) 		edge                           		node {$\chfig(set_1, 4)$} 								(enter)              
       		 	edge       [loop above]        node {$\neg \chfig(set_1, 4)$} 								(fly)
(enter) 		edge					node [below, rotate = 45]{$dir = l$} 				(hold left)
             		edge					node [fill=none,above, rotate = 45]{$\chfig(set_2, 2)$} 		(hold left)
             		edge					node [below, rotate = -45]{$dir = r$} 				(hold right)
             		edge					node [fill=none,above, rotate = -45]{$\neg \chfig(set_2, 2)$} 	(hold right)
(hold left)  	%edge	[loop above] 		node {$\neg \chfig(set_3, 1)$} 								(hold left)
             		edge					node [above,rotate = -45]{$ \chfig(set_3, 1)$} 				(base)
(base)       	edge					node {$\chfig(set_5, 1)$} 								(final app)
             		%edge	[loop above]	    	node {$\neg \chfig(set_5, 1)$} 								(base)
(hold right) 	%edge	[loop below]		node {$\neg \chfig(set_4, 1)$} 								(hold right)
             		edge					node[above, rotate = 45] {$\chfig(set_4, 1)$} 				(base)
(final app)	edge       [bend left]      	node [rectangle,draw=red,dashed,thick,  inner sep=5pt,yshift=0.4cm,xshift=-0.4cm][above, rotate = 25]  {$miss?, dir = r$} 				(hold right)
   			edge       [bend right]      	node [rectangle,draw=red,dashed,thick,  inner sep=5pt,yshift=0.2cm][above, rotate = -25] {$miss?, dir = l$}  				(hold left)
   			edge                           		node [rectangle,draw=red,dashed,thick,  inner sep=5pt, xshift=0.2cm]{$land?$} 									(runway)
%(miss left)  edge   [bend right]   node [rectangle,draw=red,dashed,thick,  inner sep=5pt,yshift=0.2cm][above]{$true$}									(hold left)
%(miss right) 	edge       [bend left]       	node[rectangle,draw=red,dashed,thick,  inner sep=5pt,yshift=0.2cm] [above]{$true$} 								(hold right)


%(land) 	 	edge     	[loop below]        	node {$true$} 										(land)  
%(runway) 	edge                           		node [above]{$true$} 								(land)

;
\end{tikzpicture}

\captionof{figure}{SATS protocol description. If a transition has updates, they show up under the arrow. \st{Idle} state not shown. \label{fig:satsfig} \nour{the states and transitions to build set5 is also not shown here..}} 

 \end{minipage}
 \end{figure*}


==> oldIntroexample.tex <==
%\input{intro-new}
%
%\section{Introduction (to be replaced)}
%%\edit{1- Strengthen references\\
%%2- Adjust the example (sec 2.1).\\
%%3- Adjust the contributions (sec 2.2)}
%
%Distributed systems, and especially distributed systems that require some form
%of consensus, are hard to build, and hard to get right.  Consequently,
%verification of distributed systems 
%%, where nodes in the network communicate via message passing, 
%is a long-standing and fruitful research area
%~\cite{Alur.AutomaticCompletionDistributed.X.2015,Alur.AutomaticSynthesisDistributed.X.2017,Alur.SynthesizingFinitestateProtocols.X.2014,Udupa.TRANSITSpecifyingProtocols.X.2013,Desai.PSafeAsynchronous.X.2013,Desai.BuildingReliableDistributed.X.2015,Wilox.Verdi.PLDI.2015,Desai.CompositionalProgrammingTesting.OOPSLA.2018,Sergey.ProgrammingProvingDistributed.POPL.2017,Deligiannis.UncoveringBugsDistributed.X.2016,Desai.DRONAFrameworkSafe.X.2017,Padon.IvySafetyVerification.PLDI.2016},
%with substantial
%efforts~\cite{Padon.PaxosMadeEPR.OOPSLA.2017,chand2016formal,lamport2002specifying,cousineau2012tla,Druagoi.PSyncPartiallySynchronous.POPL.2016,Druagoi.LogicbasedFrameworkVerifying.X.2014,Maric.CutoffBoundsConsensus.X.2017,Liu.ClarityEfficiencyDistributed.X.2012,Woos.PlanningChangeFormal.X.2016}
%in verifying intricate consensus protocols, such as
%Paxos~\cite{lamport1998part} and Raft~\cite{ongaro2014search}.
%%Unfortunately, these consensus protocols are intricate and complex, requiring
%%numerous messages to establish simple outcomes like electing a leader from a
%%set of communicating processes. 
%These efforts, however, do not directly simplify design and analysis of
%distributed applications that use consensus as merely a step in ensuring
%global properties.
%%If multiple smoke detectors sense a fire, the smoke detectors might arrive at
%%a consensus among themselves to decide which detector will send a signal to
%%the monitoring service. 
%For instance, consider a distributed smoke detector
%(Fig.~\ref{fig:introExample} shows a constituent process) whose intended
%behavior is as follows.  Upon detecting smoke, the processes coordinate using
%a consensus protocol to choose at most two processes to report the smoke to
%the fire department. More precisely, the {\em safety specification} is: (1) at
%most two processes report to the fire department and (2) processes that do not
%detect smoke do not report to the fire department.  The {\em liveness
%specification} is: if smoke was detected by some process, then the application
%eventually reports to the fire department. Thus, the application uses
%consensus as a building block to provide interesting higher-level behavior.
%
%%This distributed application may require a round of consensus to choose a
%%sensor among the sensors that detect smoke, but also contains many other
%%steps: what to do if a fire is detected, what the sensors that {\em do not}
%%detect the fire should do, what to do after the signal is sent to the
%%monitoring service, etc. The correctness properties of the system---safety
%%properties such as ``a detector that does not sense a fire does not report a
%%fire'' or liveness properties such as ``if any detector senses a fire,
%%eventually the fire is reported''---do not directly
%%reference consensus, but merely rely on the correct operation of a consensus
%%protocol.
%%
%This paper exploits the fact that numerous consensus protocols already have
%verified
%implementations~\cite{Liu.ClarityEfficiencyDistributed.X.2012,Padon.PaxosMadeEPR.OOPSLA.2017,Woos.PlanningChangeFormal.X.2016},
%and targets parameterized synthesis of distributed applications built on top
%of such verified consensus implementations. Our overall approach is based on
%{\em abstracting consensus into a primitive building block} and reasoning
%about the behavior of the rest of the application around it.
%%By doing so, a distributed application that builds on consensus can take the correctness of consensus as a
%%given, and verify the rest of the application around it. 
%
%%\mk{Cutting this for space}
%%To this end, we leverage the observation that for many applications that rely on
%%consensus to achieve some form of coherence and synchronization across
%%distributed processes, consensus effectively serves as a building block for
%%the application and can be verified separately.
%%Consider, for example, a network of smoke detectors, as one might see in an
%%IoT setting. If multiple smoke detectors sense a fire, the smoke detectors
%%might arrive at a consensus among themselves to decide which detector will
%%send a signal to the monitoring service. This distributed application requires
%%a round of consensus to choose a sensor among the sensors that detect the
%%fire, but also contains many other steps: what to do if a fire is detected,
%%what the sensors that {\em do not} detect the fire should do, what to do after
%%the signal is sent to the monitoring service, etc. And, of course, systems
%%could get even more complicated. The correctness properties of the system---safety properties
%%such as ``a detector that does not sense a fire does not report a fire'' or liveness
%%properties such as ``if any detector senses a fire, eventually a signal is
%%sent to the monitoring system''---do not directly reference consensus, but
%%merely rely on the correct operation of a consensus protocol.
%
%%Because numerous consensus protocols already have verified
%%implementations~\cite{Liu.ClarityEfficiencyDistributed.X.2012,Padon.PaxosMadeEPR.OOPSLA.2017,Woos.PlanningChangeFormal.X.2016},
%%and consensus behavior can be isolated from the rest of the application that
%%merely uses the {\em results} of consensus, we propose {\em abstracting away
%%consensus into a primitive building block.} By doing so, a distributed
%%application that builds on consensus can take the correctness of consensus as a
%%given, and verify the rest of the application around it. 
%%
%%\nour{changed this para to avoid talking about \ch as a primitive, and mention symmetry in a less formal way}\\
%As our first contribution, we introduce a simple abstraction for consensus
%protocols that can be integrated into models of distributed systems.  In this
%abstraction, the processes trying to reach consensus simply move from a global
%state where consensus would naturally start to a global state where consensus
%is achieved, using a special {\em atomic} global transition, denoted \ch.
%Such \ch transitions encapsulate the  {\em implementation details} of how
%consensus is achieved and simply provide a consistency guarantee: all
%processes that participate in the consensus round agree on the participating
%and the ``chosen'' processes.  Additionally, we define the \ch model: an
%expressive model of distributed protocols that permits \ch transitions to
%abstract consensus rounds, accommodates broadcast and rendezvous
%communication, and lends itself to symmetry-based reductions for verification.
%
%%%%%% OLD PARA %%%%%
%%This paper introduces a simple abstraction for consensus protocols that
%%can be integrated into models of distributed systems. This primitive, \ch,
%%abstracts away the %process of selecting one (or more) processes from a set of
%%%processes that are communicating. 
%%%Critically, \ch appears simply in guards on transitions, meaning that the 
%%{\em implementation details} of how consensus is
%%achieved and simply provides 
%%%correctness assumptions about the 
%%%do not factor in to the task of verifying a distributed application.
%%%While \ch appears in a process's local model (capturing, for example, the
%%%condition ``enter this state if this process is chosen''), it provides
%%distributed consistency guarantees: all processes that participate in a \ch
%%operation agree on which processes get ``chosen.'' Note that while \ch
%%directly models some basic consensus mechanisms (\eg, choosing one process
%%from a set of processes models leader election), more complicated protocols
%%%that require consensus and synchronization 
%%can be captured through one or more \ch operations.
%%%Because we want to make sure that applications that use \ch can be verified in
%%%a scalable manner, we design \ch so that it is a {\em symmetric}
%%%operation---its behavior is independent of process-specific properties like
%%%process ids. 
%%This paper defines a low-level, symmetric, {\em operational} model of distributed guarded protocols that include \ch and allow broadcast and asynchronous
%%rendezvous communication.
%
%To synthesize distributed applications described in the \ch model, this paper
%makes further contributions: {\em parameterized verification and synthesis}
%for systems in the \ch model with an {\em arbitrary} number of processes.  We
%note that parameterized verification is only decidable for restricted classes
%of distributed systems. 
%%Usually, these results restrict the verification problem
%%in at least three dimensions: i) the communication primitives a process can
%%use, ii) the network topology of the system, and iii) the supported
%%specification language. 
%For example, Esparza et al.~\cite{EsparzaFM99} showed that for (instantaneous)
%broadcast communication in a clique, safety properties are decidable, while
%liveness properties are not. Unfortunately, neither this decidability result,
%nor any other result we are aware of, is applicable to systems in the \ch
%model. 
%%that capture the coordination behavior of \ch transitions.
%
%%\milind{These paragraphs are the key new thing}
%
%Our second contribution, then, is a decidability result for parameterized
%verification w.r.t. safety properties in an extension of the broadcast model
%of Esparza et al.~\cite{EsparzaFM99}.  This extended model, called the {\em
%guarded broadcast model}, is obtained by augmenting broadcast protocols with
%additional global conditions necessary for modeling consensus. We show that we
%can map systems in our \ch model, that satisfy some conditions, to the guarded
%broadcast model, while preserving safety properties. All these results can be
%integrated to yield a semi-decision procedure for parameterized synthesis of
%systems in the \ch model, based on a parameterized verifier. 
%
%%We show that we can decide safety properties in this model, and can integrate
%%the resulting parameterized verification procedure into a semi-decision
%%procedure for parameterized synthesis.
%
%To avoid the practical challenges of parameterized verification, we make our
%third contribution: we derive {\em cutoffs} for parameterized verification for
%many interesting classes of systems in the guarded broadcast model and
%characterize the conditions under which the cutoffs hold for parameterized
%verification of systems in the \ch model.  These cutoffs enable reduction of
%parameterized verification to verification using a standard, {\em
%non-parameterized} verification engine.
%
%%\nour{can make the following more precise after section 4 is ready.}\\
%
%%`Finally, we formulate conditions under which for some classes 
%%of systems and safety properties, 
%%show how syntactic and structural constraints placed on our \ch
%%model guarantee that for some classes of protocols and safety properties, 
%%the computed cutoffs in the guarded broadcast
%%model hold in the \ch model. 
%
%All these contributions put together yield an algorithm for parameterized
%synthesis of systems in the \ch model (under certain conditions) based on a
%standard, non-parameterized CEGIS (counterexample-guided inductive synthesis)
%loop~\cite{cegis}.
%
%We build our abstractions and procedures on top of  Kinara, a recent
%verification and synthesis engine for distributed
%systems~\cite{Alur.AutomaticCompletionDistributed.X.2015,Alur.AutomaticSynthesisDistributed.X.2017,Alur.SynthesizingFinitestateProtocols.X.2014}.
%We demonstrate the utility of our \ch abstraction and cutoffs by first showing
%that several sensor network-like applications can be verified and synthesized
%by our tool. We then turn to two larger case studies: (i) the Small Aircraft
%Tracking System (SATS), a protocol for managing air traffic that requires
%several rounds of consensus between distributed processes (planes), and (ii)
%Distributed Mobile Robotics (DMR) that requires several rounds of
%synchronization to ensure that a set of distributed mobile robots generate
%action plans that do not interfere. We show that given a skeleton of the
%system we can synthesize guards that use multiple rounds of consensus to
%guarantee the correct operation of these systems.\\
%
%\subsection*{An Example} \label{sec:runningExample}
\input{introfig} 
\para{Illustrative example.} \figref{introExample} shows a finite-state, input-output machine
describing a smoke detector process from our distributed smoke detector example
from before. If there are $n$ smoke detectors, there will be $n$ instances of
this state machine. The state machine refers to the current instance using the
variable $\mathit{self}$. Each smoke detector starts in state \st{Env}. If any
detector receives the message \tr{Smoke?} from the environment, it moves to
\st{Ask}, and broadcasts \tr{DetectSmoke!!} to all other processes. Any process
still in \st{Env} when it receives the broadcast \tr{DetectSmoke??} moves to
\st{No}, where it responds to any \tr{DetectSmoke??} messages saying it did not see smoke
(\tr{Reply}$_{no}$!).
At this point, all processes that \textit{have} detected
smoke collaborate to determine who will report the incident. The self-loops on
\st{Collect} track the \tr{Reply} messages received from other processes. In the
loops between \st{Ask} and \st{Yes1} and between \st{Pick} and \st{Yes2}, 
a smoke detector process
responds to \tr{DetectSmoke??} messages with
\tr{Reply}$_{yes}$!. This enables each smoke detector to build a a set
$\mathit{participants}$ corresponding to all smoke detectors. Note that 
processes that do not see smoke respond from the \st{No} state and are not
included in
$\mathit{participants}$). Once a detector has built its participant set (i.e. $\mathit{totalReplies} = n-1$) it moves to \st{Pick}. In \st{Pick}, the detectors that detected smoke proceed to \ch at most two detectors to contact the fire department. This is the step that abstracts consensus: 
all detectors in \st{Pick} will receive a consistent view of which detectors were chosen, 
reflecting the results of a consensus protocol. 
Hence, two detectors will contact the fire department, and all the others
%, both those that did not
%detect the fire, or those that detected the fire but were not chosen to contact the fire
%department, 
move to the \st{Idle} state.
%
%
%
%
%
%
% old example:
%\noindent{\em Example.} \figref{introExample} shows a finite-state input-output
%machine describing a smoke detector process from our distributed smoke detector
%example from before. If there are $n$ smoke detectors, there will be $n$
%instances of this state machine. The state machine refers to the current
%instance using the variable $\mathit{self}$. Each smoke detector starts in
%state \st{Env}. If any detector receives the message \tr{Smoke?} from the
%environment, it moves to \st{Ask}, and broadcasts \tr{DetectSmoke!!} to all
%other processes. Any process still in \st{Env} when it receives the broadcast
%(\tr{DetectSmoke??}) moves to \st{No}, where it responds to any messages saying
%it did not see smoke (\tr{Reply}$_{no}$!). At this point, all processes that
%\textit{have} detected smoke collaborate to determine who will report the
%incident. The loop between \st{Collect} and \st{Yes} involves receiving
%\tr{Reply} messages from other processes and responding to other
%\tr{DetectSmoke} messages (with \tr{Reply}$_{yes}$!) such that each detector
%builds a set $\mathit{participants}$ that captures all detectors that saw smoke
%(those that did not see smoke respond from the \st{No} state and will not be in
%$\mathit{participants}$).
%
%Once a process has built its participant set and has responded to all other detectors that saw smoke
%(\emph{i.e.} $\mathit{totalReplies} = n-1 \land \mathit{myReplies} = \mathit{yesReplies}$), the detectors that detected smoke move to 
% \st{Pick} to \ch at most two detectors to contact the fire department. This is the step that abstracts consensus: 
%all detectors in \st{Pick} will receive a consistent view of which detectors were chosen, 
%reflecting the results of a consensus protocol. 
%Hence, two detectors will contact the fire department, and all the others
%move to the \st{Idle} state.
%
%
%
%In this setting, consensus among the detectors that saw the fire is just one
%step in a bigger system where other interesting properties should be verified that themselves do not directly reference consensus. In particular,
%the safety properties for this system are: (1) at most two detectors can contact the fire department about the fire; and (2) detectors that did not detect fire will never report
%detecting one. The liveness (progress) property is: if a fire was detected, then the system should eventually contact the fire department.

Systems of this type can be verified using our framework, and also {\em synthesized} 
to ensure the safety properties mentioned earlier.
In our experiments, we omitted the guards and updates in the dashed red boxes
and were able to synthesize the correct completions to satisfy the specification. The omitted parts
correspond to interesting questions the developer of such a system might have.
For example, 
%should the detector attempt to build a participant set of detectors that sensed a fire? 
what
should a detector do upon receiving a message from another detector? After exchanging the messages, should the detector attempt to contact the fire
department?



% \begin{figure}[htp]
%  \centering
%\includegraphics[width=0.95\linewidth]{introfig.pdf}
%\caption{A process definition of a smoke detector. Transitions are labeled
%$\act,\, g \rightarrow u$ such that $\act$ is a communication action, $g$ is a
%boolean guard and $u$ is a list of updates. An action $\act$ is of the form
%$\actname!v$ ($\actname?v$, resp.), where $\actname$ is the message label and
%$v$ is the value communicated. \textbf{fire?} is an input action from the
%environment. \textbf{Br!} $fireDet$ is an output broadcast sending $fireDet$
%to all other $n-1$ detectors while \textbf{Br}$_j? input$ is an input action
%receiving a broadcast from detector $j$ and writing the value into variable
%$input$. The bold arrow from $Wait$ to $Store$ indicates $n-1$ transitions
%each receiving a broadcast from the $n-1$ other smoke detectors.}
%\label{fig:introExample}
%\end{figure}

%\milind{Cutting this for space. I think we clearly enumerate our contributions earlier in the intro.}
%\subsection{Contributions}
%
%In summary, the contributions of this paper are:
%\begin{enumerate}
%  \item A new abstraction called \ch that abstracts away the behavior of
%  consensus protocols so that larger distributed systems that build on
%  consensus can be verified (and a proof that \ch preserves
%  symmetry, allowing systems that use \ch to be verified using symmetry-based 
%  verification engines). (\secref{choosemodel})
%  \item A decidability result of parameterized verification for
%  message-passing distributed systems that build on consensus, along with
%  cutoffs for verification. (\secref{parameterized})
%  \item Procedures and a tool for parameterized synthesis for distributed systems with consensus. (\secref{paracompsol}, \secref{implementation}).
%  %\item A tool for parameterized synthesis for distributed systems with consensus. (\secref{implementation})
%\end{enumerate}
%
%We evaluate our tool by using the cutoffs we derive to perform parameterized verification and synthesis for five case studies of applications that use consensus as a building block. (\secref{evaluation})

